MAJORITY-3SAT (and Related Problems) in Polynomial Time

Majority-SAT is the problem of determining whether an input $n$-variable formula in conjunctive normal form (CNF) has at least $2^{n-1}$ satisfying assignments. Majority-SAT and related problems have been studied extensively in various AI communities interested in the complexity of probabilistic planning and inference. Although Majority-SAT has been known to be PP-complete for over 40 years, the complexity of a natural variant has remained open: Majority-$k$SAT, where the input CNF formula is restricted to have clause width at most $k$. We prove that for every $k$, Majority-$k$SAT is in P. In fact, for any positive integer $k$ and rational $\rho \in (0,1)$ with bounded denominator, we give an algorithm that can determine whether a given $k$-CNF has at least $\rho \cdot 2^n$ satisfying assignments, in deterministic linear time (whereas the previous best-known algorithm ran in exponential time). Our algorithms have interesting positive implications for counting complexity and the complexity of inference, significantly reducing the known complexities of related problems such as E-MAJ-$k$SAT and MAJ-MAJ-$k$SAT. At the heart of our approach is an efficient method for solving threshold counting problems by extracting sunflowers found in the corresponding set system of a $k$-CNF. We also show that the tractability of Majority-$k$SAT is somewhat fragile. For the closely related GtMajority-SAT problem (where we ask whether a given formula has greater than $2^{n-1}$ satisfying assignments) which is known to be PP-complete, we show that GtMajority-$k$SAT is in P for $k\le 3$, but becomes NP-complete for $k\geq 4$. These results are counterintuitive, because the ``natural'' classifications of these problems would have been PP-completeness, and because there is a stark difference in the complexity of GtMajority-$k$SAT and Majority-$k$SAT for all $k\ge 4$.

==> leftovers.tex <==
\section{Intuition}

Given a Boolean formula $\Phi$, let $\Pr[\Phi]$ denote the probability that a random variable assignment satisfies $\Phi$. For a given $k$-CNF $\varphi$, we want to decide the truth of the inequality
 \[\Pr[\varphi] \ge \rho.\] 
We can do this by building up a special $(k-2)$-CNF $\psi$ over the same variable set, and split the probability calculation into
\[\Pr[\varphi] = \Pr[\varphi\land \psi] + \Pr[\varphi \land \lnot\psi].\]
Recalling that $\Pr[\varphi\mid\lnot\psi] \geq \Pr[\varphi\wedge\lnot\psi]$, we observe
\begin{equation}
\label{ineq:prob}
		\Pr[\varphi\land\psi]\le \Pr[\varphi]\le \Pr[\varphi\land\psi] + \Pr[\varphi\mid\lnot\psi].
\end{equation}
	%Here, the summand $\Pr[\varphi\mid\lnot\psi]$ denotes the fraction of assignments which satisfy $\varphi$ among those assignments to $\varphi$ which do not satisfy $\psi$.
	Intuitively, we will construct $\psi$ in such a way that 
	$\Pr[\varphi\mid\lnot\psi] < \eps_1$
	for an \emph{extremely} small $\eps_1 > 0$,
	so that it is possible to reduce the problem of determining $\Pr[\varphi] \geq \rho$ to the problem of determining $\Pr[\varphi\land\psi] \geq \rho$ (in other words, we reduce \thr{\rho}{$k$} on $\varphi$  to 
	\thr{\rho}{$k$} on $\varphi\land\psi$).

	This is helpful because the clauses of $\psi$ will be subclauses appearing frequently in $\varphi$, so that the formula $\varphi\land\psi$ simplifies to a a smaller equivalent formula.
	Additionally, adding the clauses of $\psi$ to $\varphi$ should make the solution space of $\varphi$ smaller, so that intuitively it becomes easier to check if the formula has fewer than a $\rho$-fraction of satisfying assignments.
	
	More precisely,  \cref{ineq:prob} shows that, if $\varphi\land \psi$ is a YES instance for \thr{\rho}{$k$}, then $\varphi$ is a YES instance as well.
	The more surprising property is that we can construct $\psi$ in such a way that, 
	if $\Pr[\varphi\land\psi] < \rho$, then (just as in our algorithm for \thr{\rho}{$3$}) we can infer that $\Pr[\varphi\land\psi] < \rho - \eps_2$ for some small $\eps_2 > \eps_1$.
	Hence by \ref{eq:prob-bound} we can deduce that $\Pr[\varphi] < \eps_1 + \rho - \eps_2 < \rho$.
	
	We construct the clauses of such a formula $\psi$ by taking cores of large sunflowers in $\varphi$. Defining what counts as ``large'' depends on quite a few parameters, so the analysis becomes rather technical. 


\section{}

%Perhaps because of this behavior, there has been some confusion in the literature about the complexity of these problems, with several works asserting intractability for \textsf{MAJ-3-SAT} and its variants.\footnote{The confusion is also likely due to the fact that the more general problem: \emph{given a $3$-CNF $F$ and integer $k \geq 0$, determine if $\#SAT(F) \geq 2^k$} is indeed $\PP$-complete. 
	%The proof follows from (a) the version of the problem for CNF formulas is $\PP$-complete, by Gill and Simon, and (b) the reduction from CNF-SAT to 3SAT preserves the number of solutions. 
	%However, the same argument cannot be used to show that $\#SAT(F) \geq 2^{n-1}$ is $\PP$-complete for $3$-CNF $F$, because the Cook-Levin reduction introduces many new variables ($n$ changes, going from CNF-SAT to 3SAT).}
%For example, the tutorial \cite{KC_MON-2-SAT-cite-talk, K_MON-2-SAT-cite} and papers \cite{GHM_MAJ-2-SAT, TM_MAJ-2-SAT, MCC_E-MAJ3SAT-NP^PP-claim} 
%claim \textsf{MAJ-2SAT} is $\PP$-complete, and 
%\cite{Mundhenk_MAJ-3-SAT, Mundhenk-thesis, KG_optimal, KG_MAJ-3-SAT, K_MAJ-3-SAT-cite} claim \textsf{MAJ-3-SAT} is $\PP$-complete.
%These claims have been used in reductions showing the proported hardness of restricted variants of Bayesian inference and maximum a~posteriori problems, which are of great interest to various communities within AI. The true complexity of MAJORITY-3SAT (and related problems) has remained a central open issue for research in these communities. %model counting and Bayesian inference.
%In 2001, Bailey, Dalmau, and Koliatis \cite{BaileyDK07} observed that the complexity of determining $\#SAT(F) \geq 2^{n-1}$ for $3$CNFs was in fact open. More recent papers have also noted that the problem was unsolved~\cite{PLMZ_open,FGL_open, CM_open}.% pointing out that \textsf{MAJ-3-SAT} is not known to be $\PP$-complete, and more recently \cite{FGL_open, CM_open} noting that it is open whether \textsf{MAJ-$k$SAT} is $\PP$-complete for any fixed positive integer $k$.

	It seems we should be able to generalize the above to ANDs of ORs of two linear equations modulo two. The idea is that ``linear independence'' will take the place of ``disjointness'' (within an OR, both equations must be linearly independent or they can be simplified). As we greedily build up the independent clause set, any clause containing equations which are dependent on the system won't get added. If the clause set is large, we should still be able to conclude NO for similar reasons; if the clause set is small, we can enumerate possible assignments to the equations, and we only have to solve $\#$SAT on linear equations modulo 2, which can be done in polynomial time. I am not sure what extra consequences arise from this result. The sat problem for this CSP is probably NP-hard...
	
	But for linear equations modulo 3, it is already NP-hard to count Boolean solutions to them, by Shafer's dichotomy theorem. (Or note that $x_1+x_2+x_3 = 1 \pmod 3$ is the same as a 1-in-3 SAT clause.)
	

\subsection{Some Thoughts}

Consider a ratio of the form $\alpha = 2^{-2^i}$ for some $i$. In the above, we are saying that an algorithm for ratio $\alpha$ implies an algorithm for ratio $\sqrt{\alpha} = 2^{-2^{i-1}}$. Thus, an algorithm for ratio $2^{-2^k}$ implies an algorithm for ratio $2^{-2^i}$ for every $i=0,\ldots,k$ (including ratio $1/2$). Of course, each time we reduce from $2^{-2^{i+1}}$ to $2^{-2^i}$, we double the number of variables from $n$ to $2n$. So, an algorithm for ratio $1/4$ on $2n$ variables can solve ratio $1/2$ on $n$ variables, and an algorithm for ratio $2^{-2^i}$ on $2^i \cdot n$ variables can solve ratio $1/2$ on $n$ variables.

So, e.g., if we decreased the ratio from $1/2$ down to $2^{-\ell}$ for $
\ell$ being a power of two, the number of variables would increase to $n(\ell-1)$. This shows that determining ratio $\geq 2^{-\sqrt{n'}}$ for an $n'$-variable formula can solve Majority SAT on about $\sqrt{n'}$ variables, for example.

Suppose we could reduce from $\alpha$ to $\alpha^2$ by only increasing variables from $n$ to $(1+\eps)n$. We could go from ratio $1/2$ down to $2^{-n}$ and only increase variables to $(1+\eps)^{\log n}\cdot n \leq n^{1+O(\eps)}$. If $\eps$ was extremely small, e.g. $1/\Theta(n)$, then we could reduce this (say) to $n+O(\log n)$. We have $n' = n+O(\log n)$ variables and we need to determine if the fraction is at least $2^{-n} \approx 2^{n'-\Theta(\log n')}$. This could be done by simply guessing polynomially many SAT assignments.



\section{Smaller Ratios are More Difficult}

We observe that the hard case of MAJSAT is when the ratio $\alpha \in (0,1)$ is small: to obtain an algorithm for ratio $\alpha \in (0,1)$, it suffices to obtain an algorithm for ratio $\alpha^2 \in (0,1)$.

\begin{theorem} Let $\alpha \in (0,1)$. Suppose we have an algorithm for determining $\text{MAJ-$k$-SAT}_{\alpha^2}$. Then we also have an algorithm for determining $\text{MAJ-$k$-SAT}_{\alpha}$. 
\end{theorem}

\begin{proof} Given a $k$-cnf $F$ on $n$ variables, make a new $k$-cnf $F'$ on $2n$ variables, defined by \[F'(x,y) = F(x) \wedge F(y).\] Observe that $\#SAT(F') = \#SAT(F)^2$, so $\#SAT(F) \geq \alpha 2^n$ if and only if $\#SAT(F') = \#SAT(F)^2 \geq \alpha^2 2^{2n}$. Hence an algorithm for determining $\text{MAJ-$k$-SAT}_{\alpha^2}$ on $F'$ immediately determines $\text{MAJ-$k$-SAT}_{\alpha}$ on $F$.
\end{proof}


\subsection{3-CSPs and 2-CSPs}

\note{Anything we get for k-SAT would immediately apply to k-CSP... so we don't really need this section...}

\begin{theorem}
Given any Boolean CSP $F$ with constraints of width at most three, we can determine in polynomial time if at least half of the assignments to $F$ are satisfying.
\end{theorem}

\begin{proof} 
Take a CSP $F$ which has arbitrary constraints of width at most three on $n$ variables. For a variable $x$, let $F_x$ be the set of constraints of $F$ containing $x$, let $F_{-x}$ be the rest. 
(We'll also want that the constraints are ``nondegenerate'', meaning roughly that every variable can affect the output... this can easily be arranged WLOG, by checking each constraint and removing any variables that can't change the output when flipped.)

If there is a ``large'' maximal disjoint set of constraints, then we can conclude NO as in the 3SAT case.

Otherwise, we have a ``small'' maximal disjoint set so we can enumerate SAT assignments to them as in the 3SAT case.

Suppose for every $x$, $F_{-x}$ contains at least one constraint. Then we can argue as before with 3SAT, to get a fast algorithm: 
\begin{itemize}
    \item If there is at least one constraint that doesn't contain $x$, we can pair it with a ``large'' maximal ``$x$-disjoint set'' (a set of other constraints involving disjoint variables) to argue that the fraction of satisfying assignments is less than $1/2$.  
    \item Otherwise for every $x$, every maximal $x$-disjoint set is ``small''. In this case, we can enumerate assignments to the constraints in these sets, get a set of constraints on one variable, and determine the counts of each of these in polynomial time.
\end{itemize}

Otherwise, suppose there is an $x$ such that $F_{-x}$ is empty ($x$ occurs in every constraint). Consider the set of 2-constraints $G_x$ and $H_x$ obtained by setting $x$ to true and false, respectively. 

\begin{itemize}
    \item If one of $G_x$ or $H_x$ is empty, then output YES if and only if the other formula is satisfiable: again this is solvable in polynomial time, because $G_x$ and $H_x$ are sets of 2-constraints so they can be encoded as 2SAT instances.

\item Otherwise, both $F_x$ and $G_x$ are nonempty. Note that we must have $\#SAT(F_x) \leq (3/4) \cdot 2^{n-1}$ and $\#SAT(G_x) \leq (3/4) \cdot 2^{n-1}$: in both constraint sets, there is at least one constraint on two variables, and it must be nondegenerate, so it has at most three out of four possible SAT assignments. Noting that $\#SAT(F) = \#SAT(G_x) + \#SAT(H_x)$, it follows that if $\#SAT(F) \geq 2^n/2$, then \emph{both} $G_x$ and $H_x$ must have \emph{at least} $1/8 \cdot 2^n$ sat assignments (because the other formula has at most $3/8 \cdot 2^n$). Therefore for both $G_x$ and $H_x$ we can run an algorithm for 2CSP that can exactly count solutions when there are $1/8 \cdot 2^n$ sat assignments (and answers NO otherwise). If the algorithm answers NO on either of $G_x$ or $H_x$, we can return NO for $F$. Otherwise, we can return the sum of $\#SAT(G_x)$ and $\#SAT(H_x)$.

\end{itemize}


\end{proof}



\section{Slightly Lower Threshold for 3-CNFs}

The proof of \Cref{thm:maj3sat} shows how, in polynomial time, we can detect if the proportion of assignments of a given 3-CNF which are satisfying is at least $1/2$.
In this section we show how to adapt this argument slightly, and check for satisfying assignments at a threshold just a bit below $1/2$.
Specifically, we prove the following result.

\begin{theorem}
\label{thm:below-maj3sat}
Set $\rho = 7/16$.
Then in polynomial time we can decide if a $3$-CNF $F$ on $n$ variables has at least $\rho 2^n$ satisfying assignments.
\end{theorem}

\note{What about fractions in $(7/16,1/2)$?}

\begin{proof}[Proof of \Cref{thm:below-maj3sat}]
We begin with some simple preprocessing to get rid of edge cases.
First, without loss of generality, we can \textbf{assume that $F$ has no duplicate clauses}. This is because if $F$ has two identical clauses, deleting one of them will not change the proportion of satisfying assignments.
Second, we may \textbf{assume that $F$ has no clauses of width 1}.
Indeed, if $F$ has such a clause, we can assign its literal to be TRUE and get a new formula $F'$ on $n-1$ variables, with the property that the fraction of satisfying assignments in $F'$ is two times the fraction of satisfying assignments in $F$. 
This is because any satisfying assignment in $F$ must assign TRUE to literals in clauses of width 1.
So we can check if $F$ has at least a $\rho$ fraction of satisfying assignments by checking if $F'$ has a $2\rho > 1/2$ fraction of satisfying assignments.
This can be done in polynomial time by \Cref{thm:maj3sat}.
Third, we can \textbf{assume no clause of $F$ simultaneously contains a variable and its negation}.
If some clause does have $x\lor\lnot x$ for some variable $x$, we can remove this part of the clause without affecting the fraction of satisfying assignments.
This either eliminates the clause or creates a clause of width 1 (at which point we're done).
Fourth and finally, we can \textbf{assume no literal is repeated in a clause} -- if some literal is repeated in a clause, we can just remove duplicates of that literal and get a smaller 3-CNF while preserving the fraction of satisfying assignments.

We now describe the algorithm. First, scan through the clauses of $F$ and check if they all share a common literal.
If they do, we can immediately report {\bf YES}, since at least a $1/2 > \rho$ fraction of the assignments (which set the common literal to be TRUE) are satisfying.

Otherwise, there is no literal that appears in every clause.
Now, scan though $F$ again and check if there exists some literal $\ell$ such that all but one clause of $F$ contains $\ell$.
Call this exceptional clause $C$.
\begin{itemize}
    \item If $C$ has width three, we immediately report {\bf YES}.
This is because, a $7/8$ fraction of assignments to the variables of $C$ satisfy the clause, and setting $\ell$ to be TRUE satisfies the remainder of the clauses. 
So in this scenario the fraction of satisfying assignments is at least $(7/8)\cdot(1/2) = 7/16 =\rho$ as claimed. 

\item Suppose instead that $C$ has width two. (Note that in this case, the argument from the previous paragraph does not work: in this case, we could only guarantee at least a $(3/4) \cdot 1/2 = 3/8 < 7/16$ fraction of satisfying assignments.) We write our 3-CNF as

    \[F = \grp{\bigwedge_{i} (\ell\lor C_i)}\land C\]
    
for some clauses of $C_i$ of width at most $2$.
Introduce the 2-CNF

    \[F' = \grp{\bigwedge_{i} C_i}\land C\]
    
on $(n-1)$ variables.

When $\ell$ is TRUE, $F$ is satisfied if and only if $C$ is satisfied.
When $\ell$ is FALSE, $F$ is satisfied if and only if $F'$ is satisfied.
So if we define
    \[s(F) = \frac{\#SAT(F)}{2^n} \quad \text{and} \quad s(F') = \frac{\#SAT(F')}{2^{n-1}}\]
to be the fractions of satisfying assignments in $F$, and $F'$, casework on the value of $\ell$ shows that

    \[s(F) = \frac 12\cdot\grp{\frac 34 + s(F')}\]
since a $3/4$ fraction of the assignments to $C$ are satisfying.
Consequently, to determine if $s(F)\ge \rho$ it suffices to check if

    \[s(F') \ge 2\rho - \frac 34 = \frac 18.\]
    
Since $F'$ is a 2-CNF, we can determine this in polynomial time by \Cref{thm:maj2sat}.
\end{itemize}

Suppose we do not fall into the above cases. Then we can now assume that for any literal $\ell$, there are at least two clauses in $F$ which do not contain $\ell$. We proceed as follows.

Go through the clauses in $F$ and extract a maximal disjoint set $S$ of clauses. 
Set the constant $b = 7$.
If $|S|\ge b$, we report {\bf NO}.
This is because the subformula determined by $S$ will have at most a $(7/8)^b < \rho$ fraction of satisfying assignments, which means $F$ does as well by 
\Cref{prop:subformula}.
To clarify: the fraction of satisfying assignments is $(7/8)^b$ if $|S| = b$ and every clause has width three, because clauses in $S$ have disjoint support. Any additional clauses in $S$ beyond the first $b$ or clauses of width one or two only serve to decrease the fraction of satisfying assignments further from this upper bound.

Otherwise, we have $|S| < b$.
We loop through all at most $7^{|S|}$ satisfying assignments $A$ of variables in $S$, and for each get an induced 2-CNF $F_{A}$ formed by replacing the variables in $S$ with the values in $A$, and deleting satisfied clauses.
For each $F_A$, we loop through its clauses of width two and extract a maximal disjoint set $S_A$.

Set  constants $b' = 10$ and $d = 6b'$.
\begin{itemize}
    \item If $|S_A| \ge d|S|$, we report {\bf NO}.
We now prove this step is correct.

By construction, every clause in $S_A$ has width two.
Moreover, $S$ was a \emph{maximal} set of disjoint clauses, so it must be dominating, in the sense that every clause in $F$ has a variable which appears in some clause of $S$.
In particular, each clause $(x\lor y)$ in $S_A$ must correspond to some clause
$(\ell\lor x\lor y)$ in $F$, where $\ell$ is a literal whose underlying variable appears in $S$. 

Since $F$ is a 3-CNF, there are at most $3|S|$ variables appearing in $S$.
Each variable can appear as itself or negated, so there are at most $2\cdot 3|S| = 6|S|$ literals whose variable appears in $S$.
Thus by averaging, there exists a literal $\ell$ such that there are at least

\begin{equation}
    \label{eq:form-ldisjoint}
    \frac{|S_A|}{6|S|} \ge \frac{d}{6} = b'
\end{equation}
    
clauses of width two in $S_A$ whose ``original'' clause in $F$ contains $\ell$.
Since $S_A$ was a disjoint set, we can write these clauses in the form

    \[C_i = (\ell\lor x_i\lor y_i)\]
    
for $1\le i\le b'$,
where the variables corresponding to the literals $x_i$ and $y_i$ are all distinct.

Recall that $F$ must have at least two clauses not containing $\ell$.
Take two such clauses $C'$ and $C''$.
We claim that the fraction of satisfying assignments for the subformula

    \[F' = \grp{\bigwedge_{i=1}^{b'} C_i} \land C'\land C''\]
    
is strictly less than $\rho$.
By \Cref{prop:subformula} this will prove that $F$ has fewer than $\rho 2^n$, which will justify the algorithm reporting {\bf NO} in this case.

Indeed, observe that if $\ell$ is TRUE, $F'$ is satisfied if and only if both $C'$ and $C''$ are satisfied.
Since we preprocessed $F$, we know that $C$ and $C''$ are distinct, nontrivial clauses of width two or three.
By inspection (i.e. brute force search over the possible formula types we could have), the maximum fraction of satisfying assignments $C'\land C''$ can have is $\gamma = 13/16$, which is achieved (for example) by 

    \[C' = a\lor b\lor c \quad \text{and} \quad C'' = a\lor b\lor d.\]
    
    \note{Interesting... how did you do this brute force? Maybe there is a more general result we can prove here?}
    
    \snote{For this I just checked it manually.
    If one of the clauses $C'$ or $C''$ has width at most $2$, the fraction of satisfying assignments is at most $3/4 = 12/16$. Otherwise, both clauses have width three, and then we can do casework on the number of distinct variables which appear in the clauses.
    ~
    If we're working with more than two clauses (or clauses of larger width) this sort of manual check is a lot less reasonable and we'd want to write a program to make this sort of argument\dots
    ~
    Even without getting the explicit upper bound of $13/16$, it made sense to me that this argument would work though, since all we need is a satisfying fraction strictly less than $7/8$. With one clause, we already have $7/8$ fraction satisfying assignments. So if we add another clause that is somehow ``not redundant'' (why I needed to preprocess $F$) then the fraction should drop.}

    
If $\ell$ is FALSE, $F'$ is satisfied only if

    \[F'' = \bigvee_{i=1}^{b'} \grp{x_i\lor y_i}\]
is satisfied.
Because the variables occurring in the $x_i$ and $y_i$ literals are all distinct, we know that $F''$ has $(3/4)^{b'}$ fraction of satisfying assignments.

Combining these observations (casework on the value assigned to $\ell$), we get that the fraction of satisfying assignments in $F'$ is at most

    \[\frac 12\cdot\grp{\frac{13}{16} + \grp{\frac 34}^{b'}} < \frac 7{16}\]
for our choice of $b' = 10$.
Thus our algorithm was correct in reporting {\bf NO}.

\item The final case we have to consider is that $|S_A| < d|S|$.
In this case, we loop through all at most $3^{|S_A|}$ satisfying assignments $A'$ of $S_A$ and for each consider the 1-CNF formula induced by taking $F_A$ and replacing the variables in $S_A$ with their assigned values.
We can then just count satisfying assignments for the resulting simple formula and add it to a running total that we keep over all choices of $A$ and $A'$.
If we terminate the process of looping through all satisfying assignments, we will have a complete count of the total number of satisfying assignments in $F$.
In this case we can just compare the total count to $\rho 2^n$ and return {\bf YES} or {\bf NO} accordingly. 
\end{itemize}


Because we go through a constant number of satisfying assignments and for each do a polynomial amount of work, the overall algorithm runs in polynomial time.
\end{proof}


\note{Can we generalize what you proved for two clauses to get something for a larger number of clauses? E.g. What's the maximum fraction of satisfying assignments for $t$ distinct (not disjoint) 3-clauses? For $k$-clauses?}

\snote{Yeah I was thinking about this too, and I don't think you can push the argument much farther as is (at least without some modification) because of the following example: take $t$ clauses of the form $(a\lor b\lor c_i)$ where the $c_i$ variables are all distinct. 
~
Then for the formula determined by these clauses is not satisfied if and only if $a, b$ are both FALSE and at least one of the $c_i$ are false. This means the fraction of assignments which are not satisfying is $(1/4)\cdot (1 - 1/2^{t})$.
In other words, the fraction of satisfying assignments is at least \[\frac 34 + \frac{1}{2^{t+2}} > \frac 34\] even though you have many distinct clauses.}

\note{I was approaching this problem by looking at the maximum size of a disjoint 3-clause set, among the set of clauses not containing $\ell$. But for $\alpha=1/4$ (for example) I still get stuck in the case where there are \emph{many} clauses containing $\ell$ and \emph{few} clauses in the disjoint clause set. In this case you still have a small hitting set for all of the 3-clauses, but in half of the cases (when $\ell$ is false) the 2-cnf has a large disjoint set.}


\section{Original Bit Argument}

\begin{lemma}
\label{lm:gen-bit-argument}
Fix a positive rational $\rho$.
Take positive integers $k\le n$.
Let $N$ be an integer which can be represented as the sum of at most $m$ integer powers of two. 
Then if 
    \[N < \rho 2^n\]
we necessarily have
    \[N \le (\rho - \eta)2^n\]
for some positive constant $\eta$ that depends only on $\rho$ and $m$.
\end{lemma}
\begin{proof}

    Write $\rho = a/b$ for some relatively prime positive integers.
    We first handle the case where $b$ is odd.
    
    If $b=1$, then $\rho = a$ is just an integer. 
    Consider the binary representation
        \[a = \sum_{i=1}^r2^{a_i}\]
    consisting of $r$ terms with exponents $a_1 > a_2 > \dots > a_r$.
    Then we can write
        \begin{equation}
        \label{eq:term-bound}
        N < \rho 2^n = \sum_{i=1}^r 2^{n+a_i}.
        \end{equation}
    
    Now, assume that $m \ge a_1 - a_r \ge r$ 
    (we can do this since increasing $m$ only expands the set of possible values for $N$).
    Define
        \[N' = \sum_{i=1}^{r-1} 2^{n+a_i} + \sum_{j=1}^{k-r+1} 2^{n+a_r-j}.\]
    We claim that $N \le N'$.
    
    Indeed, consider the binary representation of $N$.
    The inequality in \cref{eq:term-bound} implies that
    every power of two in this representation is at most $2^{n+a_1}$.
    It also implies that not all the terms $2^{n+a_i}$ appear in the binary representation of $N$, since otherwise we would have $N \ge \rho 2^n$.
    
    So, let $j$ be the minimum index such that the term $2^{n+a_j}$ does not appear in the binary expansion of $N$.
    Then we claim that other than the powers $2^{n+a_i}$ for $i < j$, no term of the form $2^{n+d}$ with $d > a_j$ can appear in the binary representation of $N$.
    This is because if such a term appeared, we would have
    
        \[N \ge \sum_{i=1}^{j-1} 2^{n+a_i} + 2^{n+d} > \sum_{i=1}^{j-1} 2^{n+a_i} + \sum_{i=j}^r 2^{n+a_i} = \rho 2^n\]
        
    since 
        \[2^{d} > \sum_{a_r\le x < d} 2^x \ge \sum_{i=j}^r 2^{a_i}.\]
        
    Using this observation, we see that if $j < r$ we immediately have $N \le N'$ since $N'$ has $2^{n+a_j}$ for all $j < r$.
    Otherwise, $j=r$.
    Then, since $N$ can be written as the sum of at most $k$ distinct powers of two, we get that
    
        \[N \le \sum_{i=1}^{r-1} 2^{n+a_i} + \sum_{x\in S} 2^x\]
    for a set $S$ of at most $k-r+1$ distinct integers each strictly smaller than $n+a_r$.
    This description makes it clear that 
        \[\sum_{x\in S} 2^x \le \sum_{j=1}^{k-r+1} 2^{n+a_r-j}\]
    which implies that $N\le N'$ as claimed.
    So if $N < \rho 2^n$, we must have
    
        \[N\le N' = \grp{\sum_{i=1}^r 2^{n+a_i}} - 2^{n+a_r} + \grp{\sum_{j=1}^{k-r+1}2^{n+a_r-j}}
        = \grp{\rho - \eta}2^n
        \]
    for
        \[\eta = 2^{a_r} - 2^{a_r - k + r - 1}\grp{2^{k-r} - 1} = 2^{a_r - 1} + 2^{a_r - k + r - 1}.\]
        
    This argument handles the case of $b = 1$.
    Now consider the case where $b$ is an odd integer greater than $1$.
    
    In this case, it is well known that $a/b$ has an infinite binary representation that is eventually periodic.
    The proof of this result follows, for example, by considering the long division algorithm on $a$ and $b$ and noting that after taking $a\bmod b$ the first time, the pigeonhole principle shows that within the first $b$ steps steps we must have a remainder modulo $b$ that repeats, which signals that the binary expansion will repeat from then on.
    For another proof, one can use Euler's totient theorem with the infinite geometric series formula.
    Regardless, we may write the binary representation
        \[\rho = \sum_{i=1}^{\infty} 2^{a_i}\]
    for an infinite sequence of integers $a_1 > a_2 > \dots$. 
    Since the denominator $b > 1$ is nontrivial, $a_i > a_{i-1} + 1$ for infinitely many indices $i$.
    Furthermore, we know there are integers $r$ and $M$ (the latter being the period of the representation) such that for all $i \ge r$, we have $a_{i} < a_{i-1} + M$.
    
    As before, assume that $m\ge r$.
    Define
        \[N' = \sum_{i=1}^m 2^{n+a_i}.\]
    We claim that if $N < \rho 2^n$ then $N \le N'$.
    
    Indeed, if $N < \rho 2^n$, every term in the binary representation of $N$ is at most $2^{n+a_1}$.
    If the terms $2^{n+a_i}$ are present in the binary representation of $N$ for all $1\le i\le m$ then $N = N'$, and there is nothing to show.
    Otherwise, let $j$ be the minimum index such that $2^{n+a_j}$ does not occur in the binary representation of $N$.
    Then other than the terms $2^{n+a_i}$ for $i < j$, $N$ cannot have a term of the form $2^{n+d}$ with $d > a_j$ in its binary representation, for otherwise we'd have $N > \rho 2^n$.
    It follows that in this case we have
    
        \[N\le \sum_{1\le i < j} 2^{n+a_i} + \sum_{i=1}^{m-j+1}2^{n+a_j - i} = \grp{\sum_{1\le i < j} 2^{n+a_i}} + 2^{n+a_{j}} - 1 < N'.\]
    Thus, we always have
        \[N\le N' = \grp{\sum_{i=1}^\infty 2^{n+a_i}} - \grp{\sum_{i > m} 2^{n+a_i}} = (\rho - \eta)2^n\]
    where 
        \[\eta = \sum_{i > m} 2^{a_i}\]
    depends only on $k$ and $\rho$.
    
    
    Finally, it remains to handle the case where $b$ is even.
    Write $b = 2^\ell c$ for some positive integer $\ell$ and odd integer $c$.
    Define $\rho' = a/c = 2^\ell\rho$.
    Then the condition that
        \[N < \rho 2^n\]
    is equivalent to the inequality
        \[N < \rho' 2^{n-\ell}.\]
    Then by applying the case when the denominator of $\rho'$ is odd, we deduce that for some $\eta > 0$ we have
    
        \[N \le (\rho' - \eta)2^{n-\ell} = (\rho - \eta/2^\ell)2^n.\]
    Since $\eta/2^\ell$ is a positive constant depending only on $\rho$ and $m$ this completes the proof of the claim.
\end{proof}


%%%% Original proof for THR-3-SAT
\section{Small Power of Two Thresholds for 3-CNFs}
\label{sec:maj3sat}


\begin{theorem}
	\label{thm:thr-pow2-3sat}
	Let $t$ be a fixed positive integer. Then given any $3$-CNF $F$ on $n$ variables, we can decide if the number of satisfying assignments of $F$ is at least $2^{n-t}$ in $n^{O(t)}$ time. ***check the time***
\end{theorem}

The problem solved in Theorem~\ref{thm:thr-pow2-3sat} almost certainly requires an exponential dependence on $t$: an algorithm running in $2^{o(t)} \cdot \poly(n)$ time for the above problem could be used to solve $\#3SAT$ in subexponential time, refuting ETH. 
\note{***Need to write this up. Idea: The reduction from Circuit-SAT on $n$ variables and $\poly(n)$ gates to 3-CNF with $\poly(n)$ variables preserves the number of SAT assignments exactly. So, determining if a 3-CNF on $n$ variables has at least $2^i$ satisfying assignments is already $\PP$-hard for appropriately chosen $i$. ***}

In our proof we will make use of the following definition.

\begin{definition}[Literal Disjoint Sets]
	Let $F$ be a CNF.
	Recall that a \emph{disjoint set} is a collection of clauses of $F$ with the property that each variable of $F$ appears in at most one of the clauses.
	For any literal $\ell$, we now define an \emph{$\ell$-disjoint set} to be a collection $S$ of clauses in $F$ with the property that $\ell$ appears in every clause of $S$, but no variable other than the one corresponding to $\ell$ appears in more than one clause of $S$.
	Sometimes we will refer to an $\ell$-disjoint set as a \emph{literal disjoint set}, leaving the value of $\ell$ implicit.
\end{definition}

We will also need the following arithmetic observation,
which will allow us to upper bound the contributions of satisfying assignments from some nicely structured subformulas.
We will use the lemma to argue that in detecting whether a CNF has enough satisfying assignments, we can avoid counting some assignments because their contributions are guaranteed to be negligible.

\begin{lemma}
	\label{lm:bit-argument}
	Take positive integers $k\le m$.
	Let $N$ be an integer which can be represented as the sum of at most $k$ integer powers of two. 
	Then if 
	\[N < 2^m\]
	we necessarily have
	\[N \le 2^m-2^{m-k}.\]
\end{lemma}
\begin{proof}
	
	Take a representation of $N$ as a sum 
	
	\[N = \sum_{i=1}^s 2^{a_i}\]
	of powers of $2$ which uses the minimum possible number of summands.
	By assumption, this representation has at most $k$ powers.
	By minimality, all the powers appearing in this representation are distinct (if there were two identical terms both equal to $2^a$, we could replace them with a single term $2^{a+1} = 2^a + 2^a$ and get a smaller representation).
	Additionally, by the assumption that $N < 2^m$ we know that every power in the representation is of the form $2^a$ for some $a < m$.
	It follows that we can bound the representation by
	
	\[N = \sum_{i=1}^s 2^{a_i} \le 2^{m-1} + 2^{m-2} + \dots + 2^{m-k} = 2^{m} - 2^{m-k}\]
	which proves the desired result. 
	
\end{proof}

\begin{definition}
	\label{def:consistent}
	A set of literals $L$ is \emph{consistent} if no two literals in $L$ are negations of one another.
	In other words, a set of literals is consistent if every literal corresponds to a distinct variable.
\end{definition}

\begin{proof}[Proof of \Cref{thm:thr-pow2-3sat}]
	First, scan through the clauses of $F$ and check if there exists a consistent set $S$ of at most $t$ literals such that every clause contains at least one of those literals. (Note this step takes $n^{O(t)}$ time.) If such a set $S$ exists, we immediately report {\bf YES}, since at least $2^{n-t}$ assignments set each of these literals to be TRUE, and any such assignment is satisfying. 
	
	Otherwise, we may assume that for every choice of $t$ consistent literals, some clause does not contain any of them.
	Call this condition $(\ast)$.
	
	Let $q = q_1 > q_2 > \dots > q_t = c$ be positive integer parameters to be specified later.
	Define $r$ to be the largest positive integer such that $r \leq t$ and there are $r$ distinct literals $\ell_1, \dots, \ell_r$ with the following property: for each index $i$, if we define $F_i$ to be the subformula of $F$ with all clauses that contain $\ell_i$ and do not contain $\ell_j$ for any $j < i$, then $F_i$ has an $\ell_i$-disjoint set of size at least $q_i$.
	(Intuitively, $r$ is the maximum number of large literal disjoint sets in $F$.) Note we can determine $r$ in in $n^{O(t)}$ time.
	
	We proceed with casework on the value of $r$.
	It will be important to pick $c$ large enough so that
	
	\begin{equation}
	\label{eq:c-bound}
	\grp{\frac{7}{8}}^c < \frac 18\cdot \grp{\frac{1}{2}}^{t}
	\end{equation}
	
	\begin{itemize}
		\item 
		Suppose $r = t$, so $r$ is as large as possible.
		Then we can immediately report {\bf NO}.
		
		Indeed, for each $i$ let $L_i$ be an $\ell_i$-disjoint set of size at least $q_i$ in $F_i$ (since $q_i$ will be a constant only depending on $t$, this can be computed in polynomial time). 
		Also, let $C$ be a clause that does not contain any of the $\ell_i$ (such a clause exists by our earlier discussion). 
		
		Let $F'$ be the subformula of $F$ consisting of all the $L_i$ and $C$.
		If any of the $\ell_i$ are set to FALSE, the resulting formula has a disjoint set of size at least $c$, and the fraction of satisfying assignments in this case is at most $(3/4)^c$.
		If all the $\ell_i$ are TRUE, at most a $7/8$ fraction of assignments  satisfy $C$.
		It follows that 
		
		\[\frac{\ssat{F'}}{2^n} \le \frac{1}{2^t}\cdot \frac{7}{8} + \grp{1 - \frac{1}{2^t}}\cdot \grp{\frac{3}{4}}^c < \frac{1}{2^t}\]
		by \cref{eq:c-bound}. 
		Then by \Cref{prop:subformula} we get that $\ssat{F} < 2^{n-t}$ as claimed.
		
		\item
		Suppose $r = 0$, so $r$ is as small as possible.
		Then we proceed by computing $\ssat{F}$ directly.
		
		Take a maximal disjoint set $S$ in $F$.
		If $|S|\ge c$ by \cref{eq:c-bound} we can immediately report {\bf NO}.
		
		So suppose $|S| < c$.
		We loop over the at most $7^{|S|}$ satisfying assignments $A$ of $S$, and for each produce a new formula $F_A$.
		Now, extract a maximal disjoint set of width-2 clauses $S_A$ from $F_A$.
		
		We claim that $|S_A|< 6q|S|$ for every $A$.
		
		Suppose to the contrary that $|S_A| \ge 6q|S|$ for some $A$.
		By maximality, $S$ is a dominating set for the clauses of $F$, so every clause in $S_A$ corresponds to a clause in $F$ with at one literal from $S$ removed.
		Since at most $6|S|$ literals could have been removed to produce the clauses of $S_A$, by averaging we deduce there is a single literal $\ell$ such that at least 
		\begin{equation}
		\label{eq:avg}
		|S_A|/6|S| \ge q
		\end{equation}
		clauses
		$(x\lor y)$ in $S_A$ pulls back to a clause $(\ell \lor x \lor y)$ in $F$.
		Hence, $F$ has an $\ell$-disjoint set of size $q=q_1$, which contradicts our assumption that $r < 1$.
		
		So, we loop over all at most $3^{|S_A|}$ satisfying assignments $A'$ of $S_A$, and for each get a 1-CNF whose satisfying assignments we can count in linear time by \Cref{prop:1cnf}. 
		We add up the counts over all $A$ and $A'$ to compute $\ssat{F}$, and then finish by checking if this count is at least $2^{n-t}$.
		
		\item
		Otherwise, $1\le r < t$.
		In this case, we consider assignments to the $\ell_i$.
		When all the literals are set to TRUE, we show how to explicitly count satisfying assignments in the induced formula.
		When one of the literals is set to FALSE, we will invoke \Cref{lm:bit-argument} and argue that the number of satisfying assignments in the resulting formula is small enough that we do not have to compute this number. 
		(Intuitively, we will reduce this case to the cases of $r=0$ and $r=t$.)
		
		As before, let $L_i$ be a maximal $\ell_i$-disjoint set of size at least $q_i$ in $F_i$ for $1\le i\le r$.
		
		Let $F'$ be the set of clauses in $F$ not contained in any of the $F_i$.
		Note that $F'$ this is nonempty by $(\ast)$. 
		
		\begin{itemize}
			\item
			If all the $\ell_i$  are set to TRUE, $F$ is satisfied if and only if $F'$ is satisfied.
			
			Take a maximal disjoint set $S'$ of $F'$.
			If $|S'|\ge c$, we can report {\bf NO} by \cref{eq:c-bound} and \Cref{prop:subformula}.
			
			So suppose $|S'| < c$.
			We loop over the at most $7^{|S'|}$ satisfying assignments $A$ of $S'$, and for each produce a new formula $F'_{A}$.
			Now, extract a maximal disjoint set of width-2 clauses $S'_A$ from $F'_A$.
			
			By the same averaging argument from \cref{eq:avg} in the previous case, we get that $|S'_A| < 6q_{r+1}|S'|$ for all $A$.
			Then by looping over the satisfying assignments of $S'_A$, counting satisfying solutions to the resulting 1-CNF, and adding them up over all $A$, we get the exact value of $\ssat{F'}$.
			Moreover, by our bounds on the disjoint sets and the proof of \Cref{prop:1cnf} we know that 
			\[N = \ssat{F'}\]
			is a sum of at most $k = 7^c3^{6q_{r+1}c} < 7^{(6q_{r+1}+1)c}$ powers of two.
			
			\item
			If at least one of the $\ell_i$ is set to FALSE, then to satisfy $F$ we need to satisfy a disjoint set of size at least $q_r$.
			This happens for an at most $(3/4)^{q_r}$ fraction of the time.
			In particular, the number of satisfying assignments in this case is at most
			
			\[\epsilon = \grp{\frac{3}{4}}^{q_r}\grp{2^n - 2^{n-r}}.\]
		\end{itemize}
		
		If the number of satisfying assignments where the $\ell_i$ are all TRUE has $N \ge 2^{n-t}$, we can immediately report {\bf YES}.
		Otherwise, we have $N < 2^{n-t}$, so by taking $m=n-t$ in \Cref{lm:bit-argument} we have
		
		\begin{equation}
		\label{eq:amplified-bound}
		N\le 2^{n-t} - 2^{n-t-k}.
		\end{equation}
		
		Thus, if we pick $q_r$ so large that we have
		
		\[\grp{\frac{3}{4}}^{q_r} < \frac{2^{n-t-k}}{2^n - 2^{n-r}}\]
		then we necessarily have
		
		\[N + \epsilon < 2^{n-t}\]
		by \Cref{eq:amplified-bound}.
		Thus we can finish by reporting {\bf NO}.
	\end{itemize}
\end{proof}


%%% Original attempt at Threshold k-SAT argument.
\section{General Thresholds for Bounded Width CNFs}

\snote{The proofs in this section are INCOMPLETE, and in the process of being modified.}

Given a positive integer $k$ and parameter $\rho \in (0,1)$, the Threshold SAT problem
\thr{\rho}{$k$} is the task of 
taking a $k$-CNF and deciding if at least a $\rho$-proportion of assignments to the formula are satisfying.
For example, \thr{1/2}{3} is precisely the \maj{3} problem discussed in \Cref{sec:maj3sat}.
We also introduce a ``greater than'' version of this problem called \thr{>\rho}{$k$}, which is the task of deciding if strictly greater than a $\rho$-fraction of assignments to a $k$-CNF are satisfying. 
In this section, we establish the complexity of these problems for constant $\rho$ and $k$ through the following two results.

\begin{theorem}
	\label{thm:thr-sat-easy}
	For any fixed positive integer $k$ and rational $\rho\in (0,1)$, the \emph{\thr{\rho}{$k$}} problem can be solved for formulas on $n$ variables in $f(k,\rho)\poly(n)$ time for some computable function $f$.
\end{theorem}

\begin{theorem}
	\label{thm:gt-thr-sat-hard}
	For any positive integer $k$ and rational $\rho\in (0,1)$,
	\emph{\thr{>\rho}{$k$}} is in \NP.
\end{theorem}

\begin{corollary}
	For all $k \geq 4$, GT-MAJ-$k$-SAT is $\NP$-complete. \\
	\note{Should also be true for all thresholds of the form $1/2^t$ as well, by a simple reduction.$c\le w$ Simply make $t$ new variables, and make $t$ copies of a given $(k-1)$-CNF formula $F$, where each copy contains a different new variable in every clause.}
\end{corollary}

\begin{corollary}
	For every $k$, there is an unbounded function $\alpha_k(n)$ and a polynomial-time algorithm which reports NO when a given $k$-CNF $F$ has less than $2^n/\alpha_k(n)$ satisfying assignments, and otherwise reports the exact number of satisfying assignments.
\end{corollary}

\Cref{thm:thr-sat-easy} is the natural generalization of \Cref{thm:thr-pow2-3sat} to CNFs of larger bounded width, and thresholds of satisfying assignments other than $1/2$.
\Cref{thm:gt-thr-sat-hard} supplements \Cref{prop:gt-maj4sat-hard} and \Cref{thm:gt-maj3sat}, by showing that \textsf{GT-}\maj{$k$} is \NP-complete if and only if $k\ge 4$.
Both of these results are proven using a structural lemma, which intuitively shows that if a $k$-CNF avoids large sunflowers with small cores, then it is equivalent to a larger depth circuit whose satisfying assignments are easy to count.

\begin{definition}
	\label{def:sunflower}
	Given a set $L$ of $c$ distinct literals, an $L$-sunflower is a set $S$ of clauses such that every clause contains the literals in $L$, and if we removed the literals of $L$ from the clause, what remains would be a disjoint set.
	We call $L$ the core, $w$ the order, and $|S|$ the size.
	
	We also use the term $c$-sunflower to generically refer to an $L$-sunflower for some set $L$ with $|L|=c$, and just ``sunflower'' to refer to a $c$-sunflower for some nonnegative integer $c$.
\end{definition}

\begin{lemma}
	\label{lm:k-cnf-disjunction-structure}
	Take $w = k-2$ and fix positive integers $Q_0, Q_1, \dots, Q_w$.
	Then there is a linear time algorithm that, given a $k$-CNF $F$, either returns a $c$-sunflower of $F$ with size at least $Q_c$ for some $c\le w$, or produces a list, whose size is bounded by a function of $k$ and the $Q_j$, consisting of
	1-CNFs such that the number of satisfying assignments in $F$ is equal to the sum of the numbers of satisfying assignments of each 1-CNF from the list.
\end{lemma}

\begin{proof}
	
	The proof proceeds by repeatedly extracting maximal disjoint sets from subformulas of $F$.
	Formally, we begin at stage $a = 0$.
	Write $\Phi_0 =\varphi_0 =  F$.
	Take a maximal disjoint set $S_0$ of $\varphi_0$.
	If $|S_0| \ge Q_0$ we return $S_0$ and halt.
	Otherwise, we have $|S_0| < Q_0 = P_0$.
	At this point $F = \Phi_0$ is a single $k$-CNF.
	
	We describe an inductive procedure that repeatedly replaces parts of $F$ with collections of smaller width CNFs.
	In general, at stage $a$ for $0\le a\le k-1$, we build a tree $\Phi_a$ of depth $a$, where nodes at level $j$ for $0\le j\le a$ are labeled by $(k-j)$-CNFs, obtained from $F$ by assigning values to some of its variables.
	In particular, the leaves of $\Phi_a$ are $(k-a)$-CNFs.
	We may identify nodes with their formulas.
	Each node will also carry a maximal disjoint set for the associated formula.
	
	Inductively, we will maintain the properties that 
	\begin{enumerate}[(i)]
		\item 
		for any $j<a$, $\Phi_j$ is identical to the tree formed by the first $j$ levels of $\Phi_a$,
		
		\item
		if a node $v$ is a child of a node $u$ in $\Phi_a$, then the formula at $v$ was obtained by assigning values to the variables in the maximal disjoint set of $u$ to the formula at $u$,
		
		\item 
		the sum of the number of satisfying assignments to the leaves of $\Phi_a$  equals $\ssat{F}$, and
		
		\item
		the size of a maximal disjoint set at any leaf node of $\Phi_a$ is bounded above by a constant depending only on the values of $a$, $k$, and $Q_j$ for $j\le a$.
	\end{enumerate}
	For the base case of $a=0$ we can verify that these properties hold.
	
	Suppose now that we are at stage $a$ for some $a \le w$, and we have the data described above.
	Take the tree $\Phi_a$, and consider any leaf node.
	Let the $(k-a)$-CNF formula at this node be $\varphi_a$ and corresponding maximal disjoint set be $S_a$.
	We loop over all at most $\grp{2^{k-a} - 1}^{|S_a|}$ satisfying assignments to variables in $S_a$, and for each assignment produce a new induced formula by setting those values in $\varphi_a$.
	Each of these formulas is added as a child of the node with $\varphi_a$.
	
	Since $S_a$ was maximal, every clause in $\varphi_a$ has a variable with a corresponding literal in $S_a$.
	So, every new formula produced in this way is a $(k-a-1)$-CNF.
	Take an arbitrary such formula $\varphi_{a+1}$ produced in this way.
	Now, extract a maximal disjoint set $S_{a+1}$ from $\varphi_{a+1}$.
	We claim that either
	\begin{equation}
	\label{eq:max-dset-growth}
	|S_{a+1}|< 2^{a+1}\frac{k!}{(k-a-1)!}Q_{a+1}\prod_{j=0}^a |S_j|
	\end{equation}
	holds regardless of the assignment to $S_a$ which produced $\varphi_{a+1}$, or we can find a literal disjoint set in $F$ of size at least $Q_{a+1}$.
	
	Indeed, suppose to the contrary that the inequality in \cref{eq:max-dset-growth} does not hold for the set $S_{a+1}$ produced by some assignment.
	Consider the unique path in the tree $\Phi_a$ from the root (node corresponding to $\Phi_0$) to $\varphi_a$.
	This path passes through nodes at levels $j=0, 1, \dots, a$.
	Let $\varphi_j$ denote the formula of the node at level $j$, and $S_j$ the associated maximal disjoint set.
	By properties (i) and (ii), we know that $\varphi_{j+1}$ was induced from the formula $\varphi_j$ by assigning values to the variables in $S_j$.
	
	Since $S_j$ is a maximal disjoint set, its variables must be a dominating set for the clauses in $\varphi_j$.
	In particular, every clause in $\varphi_{j+1}$ corresponds to a clause in $\varphi_j$ with at least one literal from $S_j$ removed.
	Because each $\varphi_j$ is a $(k-j)$-CNF, at most $2(k-j)|S_j|$ literals could have been removed to produce the clauses of $S_{j+1}$. 
	Repeatedly applying this argument, we see that there are at most
	\[\prod_{j=0}^a2(k-j)|S_j| = 2^{a+1}\frac{k!}{(k-a-1)!}\]
	choices of a set of $a$ literals which could be removed from a clause of $F$ to produce the clause $\varphi_{a+1}$.
	Then by averaging we deduce there must exist a single set $L$ of $a$ distinct literals such that 
	
	\[\frac{|S_{a+1}|}{2^{a+1}|S_0|\cdots |S_a|k!/(k-a-1)!} \ge Q_{a+1}\]
	clauses in $S_{a+1}$ which pull back to a clause containing in all the literals of $L$ in $F$
	(we are using the assumption that the inequality in \cref{eq:max-dset-growth} does not hold).
	This corresponds to an $(a+1)$-sunflower of size at least $Q_{a+1}$, so we can return this set of clauses and halt as claimed.
	We can find and return this sunflower in linear time by scanning through the clauses in $\varphi_j$ which correspond to the clauses in $S_{j+1}$ for $j=a, a-1, \dots, 0$.
	
	Otherwise, \cref{eq:max-dset-growth} holds for all assignments to $S_{a}$.
	
	By repeating this procedure for all leaves of $\Phi_a$ we produce the tree $\Phi_{a+1}$.
	Since we are merely inserting new leaves by partially assigning variables to the leaves of $\Phi_a$, properties (i) and (ii) still hold.
	
	By induction, $\ssat{F}$ equalled the sum of the numbers of satisfying assignments to the leaves of $\Phi_a$.
	In the above process, each leaf of $\Phi_a$ produced children by looping over assignments to some subset of its variables, so certainly the number of satisfying assignments at a leaf of $\Phi_a$ is equal to the total count of satisfying assignments among its children in $\Phi_{a+1}$.
	This means that property (iii) still holds.
	
	Finally, the inductive hypothesis and \cref{eq:max-dset-growth} show that property (iv) still holds.
	
	If we never produce a large sunflower,
	this process terminates once we get to $\Phi_{k-1}$.
	The leaves of this tree are 1-CNFs.
	Return the list of these leaves completes the algorithm by property (iii).
	If $M_a = M_a(k, Q_0, \dots, Q_a)$ is a bound on the size of the maximal disjoint sets of nodes at level $j$ (such a bound exists by property (iv)), then by the construction we see that the number of leaves in this tree is also bounded above by 
	\[\prod_{a=0}^w \grp{2^{k-a} - 1}^{M_a}\]
	a constant depending only on $k$ and the $Q_j$.
	Other than this constant overhead, building $\Phi_{k-1}$ simply requires extracting maximal disjoint sets for subformulas of $F$.
	Thus, this process takes linear time with respect to the size of $F$.
\end{proof}

%\begin{remark}
%	The number of $1$-CNFs produced by \cref{lm:k-cnf-disjunction-structure}
%	using the above proof gives an upper bound
%		\[\prod_{a=0}^w\grp{2^{k-a} - 1}^{2^{2^a-1}k^a(k-1)^{a-1}\cdots (k-a+1)Q_aQ_{a-1}Q_{a-2}}\]
%\end{remark}

The above lemma lets us count satisfying assignments for nicely structured subformulas.
To complement this result, we will argue that subformulas with large disjoint sets contribute a negligible number of satisfying assignments.
For this, we will need the following arithmetic observation generalizing \Cref{lm:bit-argument},


\begin{definition}
	Given an odd integer $b$, we define $\ord(b)$ to be the smallest positive integer $r$ such that 
	\[b\mid 2^r-1.\]
\end{definition}

Euler's totient theorem shows that $\ord(b)$ always exist and is a divisor of $\varphi(b) \le b-1$.
It is possible to attain this upper bound and have $\ord(b)=b-1$ if $2$ is a primitive root modulo $b$;
for example this happens whenever $b$ is a power of three.

\begin{lemma}
	\label{lm:gen-bit-argument}
	Let $\rho \in (0,1)$ be a rational with bounded numerator and denominator.
	Take positive integers $k\le n$.
	Let $N$ be an integer which can be represented as the sum of at most $m$ integer powers of two. 
	Then if 
	\[N < \rho 2^n\]
	we necessarily have
	\[N \le (\rho - \eta)2^n\]
	for some positive constant $\eta$ that depends only on $\rho$ and $m$.
\end{lemma}
\begin{proof}
	
	Write 
	$\rho = a/b$ 
	for some relatively prime positive integers.
	We first handle the case where $b$ is odd.
	
	If $b=1$, then $\rho = a$ is just an integer. 
	Consider the binary representation
	\[a = \sum_{i=1}^r2^{a_i}\]
	consisting of $r$ terms with exponents $a_1 > a_2 > \dots > a_r$.
	Then we can write
	\begin{equation}
	\label{eq:term-bound}
	N < \rho 2^n = \sum_{i=1}^r 2^{n+a_i}.
	\end{equation}
	
	Now, assume that $m \ge a_1 - a_r \ge r$ 
	(we can do this since increasing $m$ only expands the set of possible values for $N$).
	Define
	\[N' = \sum_{i=1}^{r-1} 2^{n+a_i} + \sum_{j=1}^{k-r+1} 2^{n+a_r-j}.\]
	We claim that $N \le N'$.
	
	Indeed, consider the binary representation of $N$.
	The inequality in \cref{eq:term-bound} implies that
	every power of two in this representation is at most $2^{n+a_1}$.
	It also implies that not all the terms $2^{n+a_i}$ appear in the binary representation of $N$, since otherwise we would have $N \ge \rho 2^n$.
	
	So, let $j$ be the minimum index such that the term $2^{n+a_j}$ does not appear in the binary expansion of $N$.
	Then we claim that other than the powers $2^{n+a_i}$ for $i < j$, no term of the form $2^{n+d}$ with $d > a_j$ can appear in the binary representation of $N$.
	This is because if such a term appeared, we would have
	
	\[N \ge \sum_{i=1}^{j-1} 2^{n+a_i} + 2^{n+d} > \sum_{i=1}^{j-1} 2^{n+a_i} + \sum_{i=j}^r 2^{n+a_i} = \rho 2^n\]
	
	since 
	\[2^{d} > \sum_{a_r\le x < d} 2^x \ge \sum_{i=j}^r 2^{a_i}.\]
	
	Using this observation, we see that if $j < r$ we immediately have $N \le N'$ since $N'$ has $2^{n+a_j}$ for all $j < r$.
	Otherwise, $j=r$.
	Then, since $N$ can be written as the sum of at most $k$ distinct powers of two, we get that
	
	\[N \le \sum_{i=1}^{r-1} 2^{n+a_i} + \sum_{x\in S} 2^x\]
	for a set $S$ of at most $k-r+1$ distinct integers each strictly smaller than $n+a_r$.
	This description makes it clear that 
	\[\sum_{x\in S} 2^x \le \sum_{j=1}^{k-r+1} 2^{n+a_r-j}\]
	which implies that $N\le N'$ as claimed.
	So if $N < \rho 2^n$, we must have
	
	\[N\le N' = \grp{\sum_{i=1}^r 2^{n+a_i}} - 2^{n+a_r} + \grp{\sum_{j=1}^{k-r+1}2^{n+a_r-j}}
	= \grp{\rho - \eta}2^n
	\]
	for
	\[\eta = 2^{a_r} - 2^{a_r - k + r - 1}\grp{2^{k-r} - 1} = 2^{a_r - 1} + 2^{a_r - k + r - 1}.\]
	
	This argument handles the case of $b = 1$.
	Now consider the case where $b$ is an odd integer greater than $1$.
	
	In this case, it is well known that $a/b$ has an infinite binary representation that is eventually periodic.
	The proof of this result follows, for example, by considering the long division algorithm on $a$ and $b$ and noting that after taking $a\bmod b$ the first time, the pigeonhole principle shows that within the first $b$ steps steps we must have a remainder modulo $b$ that repeats, which signals that the binary expansion will repeat from then on.
	For another proof, one can use Euler's totient theorem with the infinite geometric series formula.
	Regardless, we may write the binary representation
	\[\rho = \sum_{i=1}^{\infty} 2^{a_i}\]
	for an infinite sequence of integers $a_1 > a_2 > \dots$. 
	Since the denominator $b > 1$ is nontrivial, $a_i > a_{i-1} + 1$ for infinitely many indices $i$.
	Furthermore, we know there are integers $r$ and $M$ (the latter being the period of the representation) such that for all $i \ge r$, we have $a_{i} < a_{i-1} + M$.
	
	As before, assume that $m\ge r$.
	Define
	\[N' = \sum_{i=1}^m 2^{n+a_i}.\]
	We claim that if $N < \rho 2^n$ then $N \le N'$.
	
	Indeed, if $N < \rho 2^n$, every term in the binary representation of $N$ is at most $2^{n+a_1}$.
	If the terms $2^{n+a_i}$ are present in the binary representation of $N$ for all $1\le i\le m$ then $N = N'$, and there is nothing to show.
	Otherwise, let $j$ be the minimum index such that $2^{n+a_j}$ does not occur in the binary representation of $N$.
	Then other than the terms $2^{n+a_i}$ for $i < j$, $N$ cannot have a term of the form $2^{n+d}$ with $d > a_j$ in its binary representation, for otherwise we'd have $N > \rho 2^n$.
	It follows that in this case we have
	
	\[N\le \sum_{1\le i < j} 2^{n+a_i} + \sum_{i=1}^{m-j+1}2^{n+a_j - i} = \grp{\sum_{1\le i < j} 2^{n+a_i}} + 2^{n+a_{j}} - 1 < N'.\]
	Thus, we always have
	\[N\le N' = \grp{\sum_{i=1}^\infty 2^{n+a_i}} - \grp{\sum_{i > m} 2^{n+a_i}} = (\rho - \eta)2^n\]
	where 
	\[\eta = \sum_{i > m} 2^{a_i}\]
	depends only on $k$ and $\rho$.
	
	
	Finally, it remains to handle the case where $b$ is even.
	Write $b = 2^\ell c$ for some positive integer $\ell$ and odd integer $c$.
	Define $\rho' = a/c = 2^\ell\rho$.
	Then the condition that
	\[N < \rho 2^n\]
	is equivalent to the inequality
	\[N < \rho' 2^{n-\ell}.\]
	Then by applying the case when the denominator of $\rho'$ is odd, we deduce that for some $\eta > 0$ we have
	
	\[N \le (\rho' - \eta)2^{n-\ell} = (\rho - \eta/2^\ell)2^n.\]
	Since $\eta/2^\ell$ is a positive constant depending only on $\rho$ and $m$ this completes the proof of the claim.
\end{proof}

\begin{definition}
	\label{def:consistent-sunflower}
	A set of $c$-sunflowers with cores $L_1, \dots, L_c$ is said to be consistent if the cores are pairwise disjoint and $\cup_{i=1}^c L_i$ is consistent.
	A collection of consistent $c$-sunflowers is called a $c$-family.
\end{definition}


\begin{proof}[Proof of \Cref{thm:thr-sat-easy}]
	Take $w = k-2$.
	Set $t_0 = 0$ and 
	for $1\le c\le w$, let $t_c = \Theta(2^c\log(1/\rho))$ be the largest nonnegative integer such that
	\begin{equation}
	\label{eq:tc-bound}
	\grp{1 - \frac{1}{2^c}}^{t_c} \ge \rho.
	\end{equation}
	
	For each choice of nonnegative integers $c\le k-2$ and $j\le t_c$, we introduce a positive integer $q_{c,j}$ whose value is to be specified later.
	Intuitively, for each $c$, the constants $q_{c1} > q_{c2} > \dots > q_{ct_c}$ will determine the cutoff a $c$-sunflower to be ``large.''
	We then run the following procedure to transform $F$ and set the value of a parameter $\vec{r} = (r_0, r_1, \dots, r_w)$, where $r_c$ intuitively represents the number of large $c$-sunflowers in $F$.
	
	\begin{enumerate}
		\item 
		Initialize $F_0 = F_1 = \dots = F_w = F$ to be distinct copies of the formula $F$.
		\item 
		Initialize $r_0 = r_1 = \dots = r_w = 0$.
		
		\item
		While $r_c \le t_c$ for all $c$:
		
		\begin{enumerate}
			\item 
			Run the algorithm of \Cref{lm:k-cnf-disjunction-structure} with $Q_c = q_{c,r_c}$ .
			
			\item 
			If step 3(a) returned an $L_c$-sunflower of size at least $Q_c$ for some core $|L_c| = c$, increment the value of $r_c$ and save the sunflower.
			Let $F'$ be the set of all clauses in $F_c$ which contain all the literals in $L_c$, and replace $F_c$ with $F_c\setminus F'$. Save $F'$ as well.
			If the updated $F_c$ is empty, halt.
			
			\item
			Otherwise, step 2(a) returned a list $\Phi$ of 1-CNFs, and we halt.
		\end{enumerate}
	\end{enumerate}
	
	By \Cref{lm:k-cnf-disjunction-structure}, this routine takes linear time, viewing the $q_{c,j}$ and $t_c$ as constants.
	
	We now perform casework on the three distinct ways that this process could halt.
	
	\begin{description}
		\item[Case 1: Small Covering by Cores] \hfill\\
		The first way that the procedure could halt is that we terminate in step 3(b), because formula $F_c$ has become empty for some $c$.
		By considering how $F_c$ is updated, we see that in this case, we have identified a set of at most $t_c$ pairwise disjoint sets $L_1, \dots, L_{t_c}$ consisting of $c$ distinct literals each, such that each clause in $F$ contains the all the literals from some set $L_j$.
		Moreover, for each index $j$ we have an $L_j$-sunflower $S_j$ of size at least $q = q_{c,t_c}$.
		
		\begin{description}
			\item[Case 1(a): Overlapping Cores]\hfill\\
			Suppose two of the $L_j$ sets have a literal with the same underlying variable.
			Without loss of generality, let $L_1$ and $L_2$ share some nonempty set of variables $V$.
			In this case we immediately return {\bf NO}.
			
			Indeed, consider the $S_1$ and $S_2$ sunflowers.
			
			\item[Case 1(b): Variable Disjoint Cores]\hfill\\
		\end{description}
		
		\item[Case 1: Many Large Literal Disjoint Sets] \hfill\\
		Suppose $r = t+1$, so $r$ is as large as possible.
		Then we can immediately report {\bf NO}.
		
		\item[Case 1: Many Large Literal Disjoint Sets] \hfill\\
		Suppose $r = t+1$, so $r$ is as large as possible.
		Then we can immediately report {\bf NO}.
	\end{description}
	
	\snote{Border between new and old arguments}.
	
	At the end of this procedure, we have a nonnegative integer $r$ and $r$ distinct literals $\ell_1, \dots, \ell_r$ with the following property:
	if we define $F_i$ to be the subformula of $F$ with all clauses that contain $\ell_i$ and do not contain $\ell_j$ for any $j < i$, then $F_i$ has an $\ell_i$-disjoint set $L_i$ of size at least $q_i$ which we have access to.
	Moreover, if the procedure never produced a formula $\Phi$ (that is, we never reach step 2(c) in the algorithm), then $r=t+1$.
	Otherwise, $r\le t$ and we have a formula $\Phi$ equivalent $F\setminus \grp{\cup_i F_i}$.
	We handle these cases separately.
	
	
	\begin{description}
		\item[Case 1: Many Large Literal Disjoint Sets] \hfill\\
		Suppose $r = t+1$, so $r$ is as large as possible.
		Then we can immediately report {\bf NO}.
		
		Take the set $\ell_i$-disjoint set $L_i$ of size at least $q_i$ in $F_i$. 
		Also, let $C$ be a clause that does not contain any of the $\ell_i$, guaranteed to exist by $(\star)$.
		
		Let $F'$ be the subformula of $F$ consisting of all the $L_i$ and $C$.
		If any of the $\ell_i$ are set to FALSE, the resulting formula has a disjoint set of size at least $c$, and the fraction of satisfying assignments in this case is at most $(1 - 1/2^{k-1})^c$.
		If all the $\ell_i$ are TRUE, at most a $(1 - 1/2^k)$ fraction of assignments  satisfy $C$.
		It follows that 
		
		\[\frac{\ssat{F'}}{2^n} \le \frac{1}{2^{t+1}}\cdot \grp{1 - \frac 1{2^k}} + \grp{1 - \frac{1}{2^{t+1}}}\cdot \grp{1 - \frac{1}{2^{k-1}}}^c < \frac{1}{2^{t+1}}\]
		by \cref{eq:c-bound-general}. 
		So by \Cref{prop:subformula} we get that $\ssat{F} < 2^{n-t-1} < \rho 2^n$ as claimed.
		
		\item[Case 2: Some Large Literal Disjoint Sets] \hfill\\
		Otherwise, $0\le r \le t$.
		
		In this case, we consider assignments to the $\ell_i$.
		When all the literals are set to TRUE, we show how to explicitly count satisfying assignments in the induced formula.
		When one of the literals is set to FALSE, we will invoke \Cref{lm:gen-bit-argument} and argue that the number of satisfying assignments in the resulting formula is small enough that we may forego computing this number.
		
		As before, let $L_i$ be a maximal $\ell_i$-disjoint set of size at least $q_i$ in $F_i$ for $1\le i\le r$.
		
		Let $F'$ be the set of clauses in $F$ not contained in any of the $F_i$.
		Then $F'$ is nonempty by $(\ast)$ and equivalent to $\Phi$ by the earlier discussion.
		
		\begin{itemize}
			\item
			If all the $\ell_i$  are set to TRUE, $F$ is satisfied if and only if $F'$ is satisfied.
			Let 
			\[N = \ssat{F'} = \ssat{\Phi}\]
			be the number of satisfying assignments in this subformula.
			We compute the value of $N$ by dynamic programming on the structure of $\Phi$.
			More specifically: we count the number of satisfying assignments of each 1-CNF at the leaves of $\Phi$ by \Cref{prop:1cnf} in linear time, and get $N$ by adding all these counts up.
			Moreover, by \Cref{prop:1cnf} and the size bounds on $\Phi$ from \Cref{lm:k-cnf-disjunction-structure}, we deduce 
			that $N$ is the sum of at most $m$ powers of $2$, where $m$ is bounded above by some function depending only on $k, c$ and $q_{r+1}$.
			
			\item
			If at least one of the $\ell_i$ is set to FALSE, then to satisfy $F$ we need to satisfy a disjoint set of size at least $q_r$.
			This happens for an at most $(1 - 1/2^k)^{q_r}$ fraction of the time.
			In particular, the number of satisfying assignments in this case is at most
			
			\[\epsilon = \grp{1 - \frac{1}{2^k}}^{q_r}\grp{2^n - 2^{n-r}}.\]
		\end{itemize}
		
		If the number of satisfying assignments where the $\ell_i$ are all TRUE has $N \ge \rho 2^n$, we can immediately report {\bf YES}.
		Otherwise, we have $N < \rho 2^n$, so by \Cref{lm:bit-argument} we have
		
		\begin{equation}
		\label{eq:amplified-bound-gen}
		N\le (\rho - \eta)2^{n}
		\end{equation}
		
		where $\eta$ depends only on $\rho$ and $m$.
		
		Thus, if we pick $q_r$ so large that we have
		
		\[\grp{1 - \frac{1}{2^k}}^{q_r} < \frac{\eta 2^{n}}{2^n - 2^{n-r}}\]
		then we necessarily have
		
		\[N + \epsilon < \rho 2^{n}\]
		by \Cref{eq:amplified-bound-gen}.
		Thus we can finish by reporting {\bf NO}.
		
		
	\end{description}
	
\end{proof}

\begin{proof}[Proof of \Cref{thm:gt-thr-sat-hard}]
	
	Given a $k$-CNF $F$, we first run the polynomial time algorithm from proof of \Cref{thm:thr-sat-easy}
	to decide if at least a $\rho$ fraction of the assignments to $F$ are satisfying.
	If the algorithm returns NO then so do we.
	Otherwise, the algorithm returned YES and we know that $\ssat{F} \ge \rho2^n$.
	
	Let $t$ be the largest nonnegative integer satisfying $(1/2)^t\ge \rho$.
	Examining the proof of \Cref{thm:thr-sat-easy} we see that there are two possible ways the algorithm could return YES, which we now do casework on.
	
	\begin{description}
		\item[Case 1: Small Hitting Set of Literals] \hfill\\
		The first possibility is that there exists a consistent set $L$ of size at most $t$ such that every clause of $F$ contains at least one literal from $L$.
		In this case, the $(1/2)^{|L|}$ fraction of assignments which sets the literals in $L$ to all be TRUE are satisfying.
		
		Thus, if $t > |L|$ or $(1/2)^t > \rho$ we can immediately return {\bf YES}.
		
		If neither of these cases holds, we consider the formula $F'$ obtained from $F$ obtained by setting all the literals in $L$ to be FALSE.
		Then we nondeterministically guess a satisfying assignment for $F'$.
		If we find one, we report {\bf YES}.
		Otherwise we report {\bf NO}.
		This step is valid because it checks if there is an additional satisfying assignment beyond the $\rho 2^n$ guaranteed to exist thanks to $L$.
		
		\item[Case 2: Formula Decomposition] \hfill\\
		The remaining possibility is that the algorithm from \Cref{thm:thr-sat-easy} isolated a set of clauses $F'$ from $F$ and literals $\ell_1, \dots, \ell_r$ for some $r\le t+1$, with the property $F\setminus F'$ is precisely teh set of clauses not containing any of the $\ell_i$.
		Moreover, the algorithm will have computed the exact value of 
		\[N = \ssat{F'}\]
		and verified that $N\ge \rho 2^n$.
		
		If we actually have the strict inequality $N > \rho 2^n$ we report {\bf YES}.
		Otherwise, we loop over the $(2^r-1)$ assignments to the $\ell_i$ that do not set all the literals to TRUE, and for each nondeterminstically guess a satisfying assignment of the resulting formula induced from $F$.
		If we ever find a satisfying assignment we return {\bf YES}.
		If not, we return {\bf NO}.
		As in the previous case, thsi step is correct because we are just checking for an additional satisfying assignment beyond the $\rho 2^n$ guaranteed to exist thanks to $F'$.
	\end{description}
	
	These are the only cases where the algorithm for \thr{\rho}{$k$}-SAT will return YES.
	Since in both situations we can can decide if the fraction of satisfying assignments is strictly greater than $\rho 2^n$ using nondeterminism, \thr{<\rho}{$k$}-SAT is in \NP~ as claimed.
\end{proof}



%%% Earlier Observations

If you try and directly apply the algorithm of \Cref{thm:maj3sat} for $k$-CNFs with $k\ge 4$ (by repeatedly extracting small maximal independent sets and going through all the satisfying assignments to get smaller CNFs until you can just count solutions to a 1-CNF) you get a polynomial time algorithm that can verify whether a $k$-CNF on $n$ variables has \emph{at least} $\rho_{k-2}2^n$ satisfying assignments for $\rho_k = 1 - \frac 1{2^{k}}$.

% Case of $k=4$:

% \begin{itemize}
%     \item 
%     Solving MAJ-4-SAT seems to have more degenerate cases (or ``obstacles'') than MAJ-3-SAT (for 3-CNFs, you only need to check whether all clauses share a common literal).

%     \item
%     For example, if you can identify three literals $\ell_1, \ell_2, \ell_3$ such that every clause of a 4-CNF has at least two of these literals, you know that it is a YES instance for MAJ-4-SAT.

%     \item
%     Or, if there are two literals $\ell, \ell'$ such that every clause has $\ell\lor \ell'$ or $\lnot\ell\lor\lnot\ell'$, then we're in a YES instance for MAJ-4-SAT.
% \end{itemize}


\subsection{Earlier Claims}

% 	The work \cite{MCC_E-MAJ3SAT-NP^PP-claim} assumes that \textsf{E-MAJ-3-SAT} is complete for $\NP^\PP$ and that \textsf{MAJ-2-SAT} is complete for $\PP$.
% 	These claims are used in reductions involving certain restricted versions of maximum a posteriori problems on Bayesian Networks.

% 	The note \cite{K_MON-2-SAT-cite} claims that \textsf{MAJ-2-SAT} is $\PP$-complete to show hardness for a restricted Bayesian inference problem equivalent to the ones discussed in the previous reference.
% 	The accompanying talk \cite{KC_MON-2-SAT-cite-talk} makes the same claim.

% 	The work \cite{K_MAJ-3-SAT-cite} claims twice that \textsf{MAJ-3-SAT} is $\PP$-complete but does not explicitly use this fact.

% 	The paper and its full version \cite{BDPR_E-MAJ3SAT-NP^PP, BDPR_E-MAJ3SAT-NP^PP-full}, claim that \textsf{E-MAJ-3-SAT} is $\NP^\PP$ hard,
% 	and uses this claim to show hardness for a certain fixed point inference problem.
% 	Specifically, the paper reduces from \textsf{E-MAJ-3-SAT} to the problem of detecting if a bounded degree ``signed interaction digraph,'' a graph structure which records some data for a map from the Boolean hypercube to itself, supports a  ``Boolean network'' with multiple fixed points.
% 	The reduction from 3-CNFs seems to be used to show hardness in this bounded degree case.

% 	The work \cite{KG_MAJ-3-SAT} claims that \textsf{MAJ-3-SAT} is $\PP$-complete and \textsf{E-MAJ-3-SAT} is $\NP^\PP$ complete in an informal overview of computational complexity.

% 	The work \cite{KG_optimal} claims \textsf{MAJ-3-SAT} is $\PP$-complete and \textsf{E-MAJ-3-SAT} is $\NP^\PP$-complete.

% 	The work \cite{CDB_MAJ-3-SAT} claims that \textsf{E-MAJ-3-SAT} is $\NP^\PP$-complete.

% 	The work \cite{GHM_MAJ-2-SAT} claims that \textsf{MAJ-2-SAT} is $\PP$-complete.

% 	The work \cite{Mundhenk_MAJ-3-SAT} claims that \textsf{MAJ-3-SAT} is $\PP$-complete and \textsf{E-MAJ-3-SAT} $\NP^\PP$-complete.

% 	The work \cite{TM_MAJ-2-SAT} claims that \textsf{MAJ-2-SAT} is $\PP$-complete.

% 	The work \cite{Mundhenk-thesis} claims that \textsf{MAJ-3-SAT} is $\PP$-complete.



% The authors of \cite{FGL_open} note that is open whether \maj{$k$} is $\PP$-complete for any $k\ge 3$.
% Similarly,  points out that \maj{3} is not known to $\PP$-complete.
% More recently, \cite{} noted that the complexity of \maj{$k$} remains open for fixed $k$.


\subsection{Majority SAT for 4-CNFs}

\begin{theorem}
	\label{thm:maj4sat}
	There is a polynomial time algorithm for \maj{4}.
\end{theorem}


To prove this theorem, we will employ the following generalization of \Cref{lm:sun-3-cnf} to larger width CNFs.


If we inspect that proof, for the case of $k=4$ we can bound the function $f$ from the above lemma as

\[f(Q_0, Q_1, Q_2) < 15^{Q_0-1}7^{Q_1(4Q_0 - 3)}3^{Q_2(4Q_0 - 3)(3Q_1 - 2)} = \exp(Q_0Q_1Q_2).\]

\begin{proof}[Proof of \Cref{thm:maj4sat}]
	We begin by introducing several parameters.
	The reason for these precise choices will become clearer later in the proof,
	and for now it is enough to know that the values of these parameters are just sufficiently large constants.
	
	Let $q_0 = 11$
	be the smallest positive integer such that 
	\[(15/16)^{q_0} < 1/2.\]
	This will be the cutoff for the size of a ``large'' 0-sunflower.
	
	Let $q_1 = 21$
	be the smallest positive integer such that 
	\[(7/8)^{q_1} < \frac 1{16}.\]
	This will be the cutoff for the size of a ``large'' 1-sunflower.
	
	Set \[\gamma = \frac 12\cdot \grp{15/16 + (7/8)^{q_1}}\]
	which will be a useful upper bound for fractions of satisfying assignments in subformulas.
	Note that $\gamma$ is just a little smaller than $1/2$.
	
	Set $t' = 3$ be a positive integer such that
	\begin{equation}
	\label{eq:t-bound}
	(3/4)^{t'} \le \gamma
	\end{equation}
	and take 
	\[t = 2t'(q_1 - 1) = 126.\]
	The value of $t$ corresponds to the maximum number of large 2-sunflowers we can encounter.
	
	We also let $q_{2,r}$ for $r=1, 2, \dots, t$ be parameters to be specified later.
	The values here will correspond to our cutoffs for ``large'' 2-sunflowers.
	For now we just note that we will need $q_{2,1} > q_{2,2} > \dots > q_{2,t}$,
	and that we will take $q_{2,t} = 25$
	to be the large enough that 
	
	\begin{equation}
	\label{eq:q2-bound}
	(3/4)^{q_{2,t}} < \min\grp{1/2 - \gamma, 1/2 - (15/16)^{q_0}}
	\end{equation}
	and $q_{2,t} > q_1$.
	
	We now describe the algorithm to solve \maj{4}.
	
	Let $\varphi$ be the input 4-CNF on $n$ variables.
	By linearly scanning through $\varphi$ we can assume that no clause of $\varphi$ contains both $x$ and $\lnot x$ for any variable $x$,
	the formula contains no duplicated literals in a clause,
	and that no clause appears more than once.
	
	\begin{enumerate}
		
		%		\item 
		%		In $O(n^{q_1})$ time, check if there exists a 1-sunflower of size at least $q_1$ in $\varphi$.
		%		
		%		If there is, we halt and return {\bf YES}.
		%		
		%		\textcolor{Gray}{This is because in this case }
		
		\item 
		Initialize $F \leftarrow \varphi$ to be the input formula.
		
		Initialize $\psi \leftarrow \top$ to be a tautology, and $v\leftarrow 0$ to be the number of variables in $\psi$.
		
		\item
		For $r = 1, 2, \dots, t$:
		
		\begin{enumerate}[label=(\roman*)]
			\item 
			\label{step:trivial}
			Scan through the clauses of $F$ in linear time, and check if there exists a fixed literal occurring in every clause.
			
			If there is, halt and return {\bf YES}.
			
			\textcolor{Gray}{Note that this check returns YES if $F = \top$ is empty.}
			
			
			\item 
			\label{step:gamma}
			Check if $\ssat{\psi} \le \gamma 2^{v}$.
			
			If this inequality holds, halt and return {\bf NO}.
			
			\item 
			\label{step:sun}
			Run the algorithm of \Cref{lm:sun-k-cnf} on formula $F$ with $k=4$, $Q_0 = q_0$, and $Q_1 = q_1$, and $Q_2 = q_{2,r}$.
			
			\item
			If step 2\ref{step:sun} returns a 0-sunflower of size at least $Q_0$, halt and return {\bf NO}.
			
			\item 
			\label{step:o-sun}
			If step 2\ref{step:sun} instead returns a 1-sunflower of size at least $Q_1$,
			halt and return {\bf NO}.
			
			\item 
			\label{step:2-sun}
			If step 2\ref{step:sun} instead returns a 2-sunflower of size at least $Q_2$,
			save the sunflower $S$ and core $C$.
			
			For each of the two literals in $C$,
			check if either belongs to a 1-sunflower in $F$
			of size at least $Q_1$.
			If so, take this 1-sunflower and go back to step 2\ref{step:o-sun}.
			
			\textcolor{Gray}{The above check takes linear time for constant $Q_1$.}
			
			Otherwise, make the following updates.
			
			Update the formula $\psi \leftarrow \psi\land C$.
			Update $v$ to the be the new number of variables in $\psi$.
			
			Construct formula $F'$ by removing every clause which contains $C$ as a subclause from $F$.
			
			Update $F \leftarrow F'\land C$.
			
			\textcolor{Gray}{This update corresponds to asserting that the core $C$ is TRUE.}
			
			\item 
			Otherwise, step 2\ref{step:sun}
			returned a list of $m\le \exp(Q_0Q_1Q_2)$ 1-CNFs.
			
			Use this list to compute the fraction of satisfying assignments in $F$. 
			
			If this fraction is at least $1/2$ halt and return {\bf YES}.
			Otherwise halt and return {\bf NO}.
			
		\end{enumerate}
		\item 
		If the loop completed without halting, we scan through the clauses of $F$ and check if there is a single literal hitting every clause.
		
		If there is, halt and return {\bf YES}.
		
		Otherwise, halt and return {\bf NO}.
	\end{enumerate}
	
	We now prove correctness of the above algorithm.
	The high-level idea of our proof is to bound $\ssat{\varphi}$ by conditioning
	on whether $\psi$ is satisfied or not.
	
	Suppose $r-1$ iterations of the loop have completed so far.
	Then prior to entering the loop for the $r^{\text{th}}$ time, we will
	have so far discovered a sequence of clauses $\set{C_i}_{1\le i < r}$ of width exactly
	two and a sequence of formulas $\set{F_i}_{1\le i \le r}$ such that 
	
	\begin{itemize}
		\item 
		$F_1 = \varphi$		
		\item 
		$F_{i}$ contains a 2-sunflower of size $q_{2,i}$ with core $C_i$, 		
		\item
		the set of satisfying assignments of $F_{i+1}$ is precisely the set of satisfying assignments of $F_i \land C_i$, and
		\item 
		the 2-CNF $\psi = C_1 \land \dots \land C_{r-1}$ is satisfied by more than a $\gamma$ fraction of its assignments
	\end{itemize}
	for indices $1\le i < r$.
	Note that $F = F_{r}$ when we enter the loop on iteration $r$.
	The last bullet point holds true because it is true initially when $\psi = \top$,
	and then holds inductively by the check in step 2\ref{step:gamma}.
	
	An easy induction argument with the first and third bullet point above shows that the satisfying assignments of $F_r$ are precisely the satisfying assignments of $\varphi\land \psi$.
	
	Given a Boolean formula $F$, let $\Pr[F]$ denote the probability a random assignment of values to its variables is satisfying (i.e.  the fraction of satisfying assignments of $F$).
	Then we evidently have 
	\begin{equation}
	\label{eq:total-prob}
	\Pr[\varphi] = \Pr[\varphi\land \psi] + \Pr[\varphi\land \lnot\psi] = \Pr[F_r] + \Pr[\varphi\land \lnot\psi].
	\end{equation}
	
	From this equation, we can immediately make the following observation.
	\begin{claim}
		\label{claim:yes-case}
		If $\ssat{F_r} \ge (1/2)2^n$, then at least half the assignments of $\varphi$ are satisfying.
	\end{claim}
	\begin{proof}
		In this situation, \cref{eq:total-prob} implies that
		\[\Pr[\varphi] \ge \Pr[F_r] \ge 1/2\]
		as claimed.
	\end{proof}
	
	To help identify cases where we can report NO, we also note the following result.
	
	\begin{claim}
		\label{claim:no-case}
		Among assignments to $\varphi$ which do not satisfy $\psi$,
		the fraction which are satisfying for $\varphi$ is at most
		
		\[(3/4)^{q_{2,r-1}} < 1/2 - \gamma.\]
	\end{claim}
	\begin{proof}
		Each $F_i$ contains a 2-sunflower with core $C_i$.
		If $\psi$ is not satisfied by an assignment, there is a minimum index $i$ for which $C_i$ evaluates to FALSE.
		In the case where such a $C_i$ is false, we must satisfy a maximal disjoint set of size of at least $q_{2,i}$, so by 
		so by \Cref{prop:subformula} the fraction of assignments in this case is bounded above by
		\[(3/4)^{q_{2,i}} < (3/4)^{q_{2,r-1}} < 1/2 - \gamma\]
		by our choice of parameter in \cref{eq:q2-bound}.
		This holds for all cases, so the overall probability bounds holds.
	\end{proof}
	
	With these observations, we now show that our algorithm always reports the correct result.
	
	\begin{description}
		\item[Halting at Step2(i)]\hfill\\
		
		In this case, every clause of $F_r$ has a common literal.
		Consequently, any assignment which sets that literal to TRUE will satisfy $F_r$.
		At least half of the assignments to the variables satisfy this property, so
		by \Cref{claim:yes-case} we can report {\bf YES}.
		
		\item[Halting at Step 2(ii)] \hfill\\
		
		If $\ssat{\psi} \le \gamma 2^v$,
		then we certainly have
		\[\Pr[\varphi\land \psi] \le \Pr[\psi] \le \gamma.\]
		By \Cref{claim:no-case} we may also bound
		\[\Pr[\varphi\land \lnot \psi] \le \Pr[\varphi \mid \lnot \psi ] < 1/2 - \gamma.\]
		Then if we add these two inequalities together,
		by \cref{eq:total-prob} we have 
		\[\Pr[\varphi] < \gamma + (1/2 - \gamma) = 1/2\]
		so we can report {\bf NO}.
		
		\item[Halting at Step 2(iv)] \hfill\\
		
		In this case, $F_{r}$ has a 0-sunflower $S$ of size at least $q_0$.
		So by \Cref{prop:subformula} its fraction of satisfying assignments is at most $(15/16)^{q_0}$.
		So by \cref{eq:total-prob} and \Cref{claim:no-case} we have 
		
		\[\Pr[\varphi] \le \Pr[F_r] + \Pr[\varphi\mid\lnot\psi] \le (15/16)^{q_0} + (3/4)^{q_{2,t}} < 1/2\]
		by our choice of $q_{2,t}$ in \cref{eq:q2-bound}.
		Thus we can report {\bf NO}.
		
		\item[Halting at Step 2(v)] \hfill\\
		
		In this case, $F_{r}$ has a 1-sunflower $S$ of size at least $q_1$.
		Let $\ell$ be the literal in the core of this sunflower.
		We already passed the check in step 2\ref{step:trivial},
		so there must exist some clause $C$ in $F_r$ which does not contain $\ell$.
		If we take the subformula of $F_r$ consisting of $S$ together with $C$,
		casework on the value assigned to $\ell$ shows that the fraction of satisfying assignments for this subformula is at most 
		
		\[\frac 12\cdot\grp{(15/16) + (7/8)^{q_1}} = \gamma.\]
		
		By \Cref{prop:subformula} the above is an upper bound on the fraction of satisfying assignments in $F_r$ as well.
		So again by \cref{eq:total-prob} and \Cref{claim:no-case} we have 
		\[\Pr[\varphi] \le \Pr[F_r] + \Pr[\varphi\mid\lnot\psi ] < \gamma + (1/2 - \gamma) = 1/2\]
		and we can report {\bf NO}.
		
		\item[Halting at Step 2(vii)] \hfill\\
		
		In this case, we can compute the number of satisfying assignments 
		in each of the 1-CNFs in
		linear time using \Cref{prop:1cnf}.
		Adding up these counts lets us compute
		
		\[N = \ssat{F_r}\]
		
		as an integer which is the sum of at most $m$ powers of two,
		where $m$ is the number of 1-CNFs in the list.
		If $N \ge 2^{n-1}$, by \Cref{claim:yes-case} we can return YES.
		
		Otherwise $N < 2^{n-1}$,
		so by \Cref{lm:gen-bit-argument} and case 1 of \Cref{rm:examples}
		we get that 
		
		\[N \le 2^{n-1} - 2^{n-m-1}.\]
		
		Then substituting this into \cref{eq:total-prob} and applying
		\Cref{claim:no-case}
		we get that 
		
		\[\Pr[\varphi] \le \Pr[F_r] + \Pr[\varphi\mid\lnot\psi]
		\le (1/2 - 1/2^{m+1}) + (3/4)^{q_{2,r-1}} < 1/2\]
		
		as long as we take $q_{2,r-1}$ large enough that
		
		\[(3/4)^{q_{2,r-1}} < (1/2)^{m+1}.\] 
		
		By construction we have $m\le \exp(q_0q_1q_{2,r})$
		(recall we are using $\exp(A)$ to denote a quantity that is $O(2^A)$),
		so for some large enough choice of $q_{2,r}$ with
		
		\[q_{2,r-1} \le \exp(q_{2,r})\]
		
		the previous bound holds and we can report {\bf NO}.
		
		\item[Halting at Step 3] \hfill\\
		
		If $F_t$ has a single literal hitting all its clauses,
		similar reasoning to the case where we halt in step 2\ref{step:trivial}
		shows that we can report {\bf YES}.
		
		Otherwise,  assume there is no single literal that hits all the clauses of $F_t$.
		
		If none of the previous cases occurred,
		then we halt after going through the loop $t$ times.
		This means that $\psi$ consists of $t$ clauses of width 2.
		
		Whenever we added a clause $C$ to $\psi$, we removed all appearances of $C$ as a subclause in $F_r$.
		So, no formulas $F_r$ can have $C$ as the core of a large 2-sunflower (since our cutoff for a large 2-sunflower is strictly greater than 1).
		Thus, the clauses in $\psi$ are all distinct.
		
		We claim that the fraction of satisfying assignments in $\psi$ is at most $\gamma$.
		We prove this by leveraging the following observation.
		
		\begin{claim}
			\label{claim:few-repeats}
			Any literal $\ell$ appears fewer than $q_1$ times in $\psi$.
		\end{claim}
		
		For this claim to hold, we will need to make our parameters for sizes of 2-sunflowers grow quickly enough, in the sense that we have 
		
		\begin{equation}
		\label{eq:qsum-bound}
		q_{2,r-1} \ge q_1 + 4\grp{\sum_{r\le j \le t} q_{2,j}}
		\end{equation}
		
		for all $r\ge 2$, and $q_{2,t} > q_1$.
		This already holds for some $q_{2,r-1} \le \exp(q_{2,r})$ as we chose earlier.
		
		\begin{proof}
			Suppose to the contrary that literal $\ell$ appears $q_1$ times in $\psi$.
			Let $C_1, C_2, \dots, C_{q_1}$ be the first $q_1$ clauses with $\ell$,
			going from latest clause added to earliest clause added.
			
			We can write $C_i = (\ell\lor \ell_i)$ for some distinct literals $\ell_i$.
			Let $S_i$ denote the 2-sunflower in $\varphi$ that $C_i$ was the core of.
			We assume $S_i$ was taken at iteration $r_i$ of the loop, and thus has size at least $q_{2,r_i}$.
			
			Take a clause $D_1$ from $S_1$ not containing any $\ell_i$ for $i > 1$.
			Such a clause exists because we assumed that
			and $q_{2,r_1} \ge q_{2,t} \ge q_1$,
			and $S_1$ is a 2-sunflower so the $\ell_i$ can appear in at most $q_1 - 1$ clauses of $S_1$.
			
			Besides the literals in core $C_1$,
			$D_1$ has at most two other literals.
			
			Neither of these literals can be one of the $\ell_i$ appearing in the selected cores.
			This is because if $D_1$ contained $\ell_i$ for some $i > 1$,
			then it means $D_1$ has $C_i$ as a proper subclause.
			But when we added $C_i$ to $\psi$ in step 2\ref{step:2-sun}, we removed all clauses containing $C_i$ as a subclause, so it would be impossible for $C_1$ to contain it later (since $C_i$ was added to $\psi$ before $C_1$ by assumption).
			Save the clause $D_1$.
			
			By the above discussion and the fact that $S_2$ is a 2-sunflower, 
			at most $4q_{2,r_1}$  clauses of $S_2$ share a variable
			with the literals in $D_1\setminus C_1$.
			Then by \cref{eq:qsum-bound}, we know that the (potentially weaker) inequality
			
			\[q_{2,r_2} \ge q_{2, r_1} + 4q_{2,r_1}\]
			holds, which means that we can take some clause $D_2$ from $S_2$ with the property that $D_2\setminus C_2$ has no literal $\ell_i$ with $i\neq 2$,
			and $(D_2\setminus C_2)$ together with $(D_1\setminus C_1)$ form a variable disjoint set.
			
			If we repeat this argument for each index $i$ and appeal to \ref{eq:qsum-bound},
			we can extract a single clause $D_i$ from each $S_i$ such that 
			the set $D$ of clauses $D_1, \dots, D_{q_1}$ form a 1-sunflower with core $\ell$.
			
			Then $D$ is a 1-sunflower of size $q_1$ that would have existed in the subformula when the sunflower $S_{q_1}$ with core $C_{q_1}$ was first found.
			But at that point, step 2\ref{step:2-sun} would have found this 1-sunflower and halted.
			This contradicts our assumption that the routine completed all $t$ iterations of the loop, and the claim holds.		
		\end{proof}
		
		So, $\psi$ is a 2-CNF where every clause has width two and every literal $\ell$ shows up at most $q_1 - 1$ times.
		Because we took $t = 2t'(q_1 - 1)$, the formula $\psi$ must have a disjoint set of size at least $t'$.
		Then by our choice of $t'$ satisfying \ref{eq:t-bound} and \Cref{prop:subformula}, 
		we deduce that the fraction of satisfying assignments in $\psi$ is at most $\gamma$.
		
		Thus, applying \cref{eq:total-prob} together with \Cref{claim:no-case} as in previous cases we get that 
		
		\[\Pr[\varphi] \le \Pr[\psi] + \Pr[\varphi\mid\lnot\psi ] < \gamma + (1/2 - \gamma) = 1/2\]
		
		so we can report {\bf NO}.	
	\end{description}	
	
	This verifies correctness of all halting states of the algorithm, and proves that the algorithm succesfully solves the \maj{4} problem.
	The only procedures we employ are scans through subformulas of $\varphi$,  calls to \Cref{lm:sun-k-cnf}, and checking for 1-sunflowers of size at least $q_1$ with a given core.
	Each of these steps is repeated at most $t = O(1)$ times.
	
	Scanning through clauses in a subformula only takes linear time.
	The calls to \Cref{lm:sun-k-cnf} also take linear time,
	but the constant hidden in the $O(|\varphi|)$ notation is galactic,
	since it is $\exp(q_{2,1})$ where $q_{2,1}$ is itself a tower of exponentials of height $t$.
	Checking for a 1-sunflower of size at least $q_1$ takes linear time for constant $q_1$ using the algorithm of \cite{fpt-mset-packing} for example.
	
	So overall the algorithm runs in linear time, since all are parameters are constants whose values do not depend on the size $|\varphi|$ of the input 4-CNF.
\end{proof}


	

\begin{remark}
	In the above proof, at each stage we selected maximal variable disjoint sets consisting of the clauses with some fixed length.
	If instead we took maximal variable disjoint sets with no restriction on the width of the clauses picked, the proof would still work.
	All that would change is the averaging argument would be a little different, because between stages it is possible that a clause would lose strictly more than one literal.
	It is  possible this alternate version could me more useful for certain applications.
\end{remark}

\section{Arithmetic Lemma}
\label{sec:bit}


\begin{proof} Let $\rho = a / (2^v b)$ be given. We first handle the case where $b=1$, so that $\rho = a/2^v$ is a dyadic rational.
	
	{\bf Case 1: $b=1$.~ \\} For a positive integer $a$, let $a_i$ be such that \[a = \sum_{i=1}^s 2^{a_i}\]
	consisting of $s$ terms with exponents $a_1 > a_2 > \dots > a_s$.
	Then we have
	
		\begin{equation}
		\label{eq:binary-bound}
		N < \rho 2^n = \sum_{i=1}^s 2^{n-v+a_i}.
		\end{equation}
	
	By assumption, $N$ is the sum of at most $m$ powers of two.	
	Without loss of generality, suppose $m \ge s$ (this is fine, since setting $m$ to be larger only weakens the hypothesis).
% 	\note{Since you wrote ``at most $m$'' in the lemma statement, couldn't you always set $m$ to be larger? Not sure why you need case splitting here. Maybe you meant that $N$ is the sum of exactly $m$ powers of two?}
% 	{\bf Case 1(a): $b=1$ \& $m < s$.~ \\}	In this subcase set
% 		\[N' = \sum_{i=1}^m 2^{n-v+a_i}.\]
% 	We claim that $N\le N'$.
	
% 	Indeed, the inequality \cref{eq:binary-bound} shows that the powers of two showing up
% 	in the	binary representation of $N$ are all at most $2^{n-v+a_1}$.
% 	Let $j$ be the minimum index such that the term $2^{n-v+a_j}$ does not appear in the binary expansion of $N$.
% 	Such a $j$ exists because $m < s$, and in fact we must have $j\le m$ since $N$ is a sum of at most $m$ powers of two.
% 	The we claim that besides powers $2^{n-v+a_i}$ for $i<j$,
% 	no term of the form $2^{n-v+d}$ with $d > a_j$ can appear in the binary expansion of $N$.
	
% 	This is because if $d > a_j$ we have
	
% 		\[2^d \ge 2^{a_j+1} > \sum_{i=j}^s 2^{a_i}\]
% 	so if $N$ had such a term in its binary expansion we would have
	
% 		\[N\ge \grp{\sum_{1\le i < j}2^{n-v+a_i}} + 2^{n-v+d} > \sum_{i=1}^s 2^{n-v+d}\]
% 	which contradicts \cref{eq:binary-bound}.
	
% 	Hence if $j < m$ we have $N < N'$ and if $j = m$ we have $N = N'$.
% 	Thus in this subcase we have 
	
% 		\[N\le N'  = (\rho - \eta)2^n\]	
% 	for
% 		\begin{equation}
% 		\label{eq:eta-1a}
% 		\eta = \sum_{m< i \le s} 2^{a_i-v} = \frac{a - 2^{a_m}\lfloor a/2^{a_m} \rfloor}{2^v}.
% 		\end{equation}
	
% 	Qualitatively, the value of $\eta$ tends to be larger for larger values of $a$,
% 	while the ratio $\eta/\rho$ tends to be larger when $a_m - a_{m+1}$ is smaller (i.e. when $a$ has small gaps between the ones in its binary representation).
	
% 	{\bf Case 1(b): $b=1$ \& $m \ge s$~ \\}
	
% 	The proof here is nearly identical to the previous subcase.
% 	In this subcase set
Set
	
		\[N' = \sum_{i=1}^{s-1} 2^{n-v+a_i} + \sum_{j=1}^{m-s+1}2^{n-v+a_s-j}.\]
		
	We claim that $N\le N'$.
	
	Indeed, the inequality \cref{eq:binary-bound} shows that the powers of two showing up
in the	binary representation of $N$ are all at most $2^{n-v+a_1}$.
Also, not all the terms $2^{n-v+a_i}$ can show up in the binary representation,
since then we would have $N \ge \rho 2^n$.

So let $j$ be the minimum index such that the term $2^{n-v+a_j}$ does not appear in the binary expansion of $N$.
The we claim that besides powers $2^{n-v+a_i}$ for $i<j$,
no term of the form $2^{n-v+d}$ with $d > a_j$ can appear in the binary expansion of $N$.

This is because if $d > a_j$ we have

\[2^d \ge 2^{a_j+1} > \sum_{i=j}^s 2^{a_i}\]
so if $N$ had such a term in its binary expansion we would have

\[N\ge \grp{\sum_{1\le i < j}2^{n-v+a_i}} + 2^{n-v+d} > \sum_{i=1}^s 2^{n-v+d}\]
which contradicts \cref{eq:binary-bound}.

This already shows that if $j < s$ we have $N < N'$.
Otherwise $j = s$, and the assumption on $N$ implies that 

	\[N \le \sum_{i=1}^{s-1} 2^{n-v+a_i} + \sum_{x\in X} 2^x\]
for some set $X$ of $m-r+1$ distinct integers each smaller than $n-v+a_r$.
But any such set satisfies

	\[\sum_{x\in X} 2^x \le \sum_{j=1}^{m-s+1} 2^{n-v+a_s-j}\]
which means that $N\le N'$ as claimed.
	
	Thus in this subcase we have 
	
	\[N\le N' = (\rho - \eta)2^n \]
	for 
	
	\begin{equation}
	\label{eq:eta-1b}
	\eta = \frac{2^{a_s- m + s- 1}}{2^v}.
	\end{equation}
	
	The above arguments prove the result if $b = 1$.
	It remains to handle the case where $b > 1$ is an odd integer.
	
	{\bf Case 2: $b>1$~ \\}
	
	Let $d = \ord(b)$ and set $c = \grp{2^d - 1}/b$.
	Then we have
	
		\[\rho = \frac{a}{2^vb} = \frac{ac}{2^v\grp{2^d-1}}.\]
		
	Write $ac = \grp{2^d-1}q + r$ for some unique choice of nonnegative integers $q$ and $r$ with $r < 2^d-1$.
	Then we can further simplify
	
		\begin{equation}
		\label{eq:rho-bin-split}
		\rho = \frac{1}{2^v}\cdot \grp{q + \frac{r}{2^d-1}}.
		\end{equation}
	It may be helpful to think of $q$ and $r$ respectivly as the integer and fractional parts
	of $a/b$.
		
	Now take the binary representations
	
		\[q = \sum_{1\le i \le s} 2^{q_i}\quad
		\text{and}
		\quad
		r = \sum_{1\le i\le t} 2^{r_i}\]
	for nonnegative integers $q_1 > \dots > q_s$ and $d > r_1 > \dots > r_t \ge 0$.
	Note that if $q=0$ we have $s=0$ so that the first sum above can be empty.
	Using the formula for an infinite geometric series we can expand
	
		\[\frac{r}{2^{d}-1} = \grp{\sum_{1\le i\le t} 2^{r_i}}\grp{\sum_{j\ge 1} 2^{-jd} }
		= \sum_{j=1}^\infty \sum_{i=1}^t 2^{r_i - jd}.\]
		
	So if we define the infinite sequence $a_1 > a_2 > \dots$ of integers by taking
	$a_i = q_i$ for $i\le s$ and 
		\[a_{s+tj+i} = r_i-jd\]
	for all nonnegative integers $j$ and $1\le i\le t$,	
	substituting these binary expansions into \cref{eq:rho-bin-split}
	yields
	
		\[\rho = \sum_{i=1}^{\infty} 2^{a_i-v}.\]
		
	For this case, set 
	
		\[N' = \sum_{i=1}^m 2^{n-v+a_i}.\]
		
	As before, we claim that $N\le N'$.
	
	Since $N < \rho 2^n$,
	the binary expansion for $\rho$ shows that the terms in the binary expansion of $N$ are each at most $2^{n-v+a_1}$.
	If for all $1\le i\le m$ the term $2^{n-v+a_i}$ shows up in the binary expansion of $N$, then $N=N'$ and the claim holds.
	Otherwise there is some minimum index $j$ such that $2^{n-v+a_j}$ does not occur in the binary expansion of $N$.
	We cannot have a term of the form $2^{n-v+d}$ with $d > a_j$ in the binary representation of $N$, since then we'd immediately get $N > \rho 2^n$.
	So in this case
	
	        \[N\le \sum_{1\le i < j} 2^{n-v+a_i} + \sum_{i=1}^{m-j+1}2^{n+a_j - i} < N'.\]
	        
	Thus in this case too we have
	
		\[N\le N' = (\rho - \eta)2^n\]
		
	for
		
	\begin{equation}
	\label{eq:eta-2}
	\eta = \sum_{i=m+1}^\infty 2^{a_i - v}.
	\end{equation}
%	For additional context, when $m\le s$ the above equality can be written as 
%	
%		\[\eta =  \frac{q - 2^{q_m}\lfloor q/2^{q_m} \rfloor}{2^v} + \frac{r}{2^v\grp{2^d-1}}\]
%	
%	If instead $m > s$ the above equality looks like 
%	
%		\[\eta = \dots + \frac{r}{2^{v+d\lfloor(m-s)/t\rfloor}\grp{2^d-1}}\]
\end{proof}



	The value of $\eta$ obtained in \Cref{lm:gen-bit-argument} depends 
	in a somewhat complicated fashion 
	on the binary representations of the numerator and denominator of $\rho$, as
	detailed in equations \cref{eq:eta-1a}, \cref{eq:eta-1b}, and \cref{eq:eta-2}.
	To get some intuition for how big these gaps are, here are the precise bounds we obtain for
	$\eta$ for some concrete choices of $\rho$:
	
		\begin{enumerate}
			\item 
			When $\rho = 1/2^v$ is the inverse of a power of two, \cref{eq:eta-1b} shows that 
				\[\eta = \frac{\rho}{2^m}.\]
				
			\item 
			When $\rho = 3/7$, simplifying the expression in \cref{eq:eta-2} shows that
				\[\eta = \frac{\rho}{2^{3m/2}}\]
			when $m$ is even and 
				\[\eta = \frac{(5/3)\rho }{2^{\lceil 3m/2\rceil }}\]
			when $m$ is odd.
			
			The decay is worse in terms of $m$ than in the previous case 
			because the denominator has nontrivial order $\ord(7) = 3 > 1$.
				
			\item 
				When $\rho = 1/2 - 1/2^{v}$, for $m < v-1$ we can compute 
									\[\eta = \frac{1}{2^{m+1}} - \frac{1}{2^v} \]
				by \cref{eq:eta-1a}.
									
				If instead $m \ge v-1$, we can compute from \cref{eq:eta-1b} that
					\[\eta = \frac{1}{2^{m+2}}.\]
					
				So for $m \ge v-1$ the behavior in this case is similar to
				what happens when $\rho = 1/2$,
				but if $v$ is much bigger than $m$ we potentially then there can be some ``extra loss'' in the gap $\eta$.
						
			\item 
		When $\rho = 1/3^v$ is the inverse of a power of three, \cref{eq:eta-2} implies that 
		\[\eta \ge  \frac{\rho }{2^{2\cdot 3^{v-1}\lceil m/h\rceil }}\]
		
		where $1\le h < 2\cdot3^{v-1}$ is the number of ones in the binary expansion of $(4^{3^{v-1}}-1)/3^v$.
		
		Like the previous examples, the decay is exponential in $m$.
		However, here the decay is much more rapid in terms of $v$.
		The seems to be representative of a worst case scenario where the denominator of $\rho$ has two as a ``primitive root.''
		
		\item 
		When $\rho = 1/(2^v-1)$, \cref{eq:eta-2} implies that 
			\[\eta = \frac{\rho}{2^{mv}}.\]
		Note that this decay is much more rapid than in the first example
		where $\rho = 1/2^v$, even though the threshold values themselves are close.
		\end{enumerate}




\begin{remark}
	\label{rm:c3-note}
	If we restrict our attention to $\rho = 1/2^t$ for some positive integer $t$
	(or even $\rho$ between $(1/2)^t$ and $(7/8)(1/2)^t$)
	the argument for {\bf case 3} in the proof of \Cref{thm:thr-3-sat} can be
	made simpler.
	Currently, for general $\rho$, we need to run the loop for up to $(t+1)$ steps and argue that 
	if we get $(t+1)$ sunflowers of weight $1$, the total fraction of satisfying assignments is too small.
	
	However, when $\rho = 1/2^t$, it suffices to run the loop with test $r < t$ 
	(so that it runs for up to $t$ steps): if the while loop exits without early termination, then we must have $t$ 1-sunflowers and a nonempty subformula left over.
	Since the fraction of satisfying assignments in this remaining subformula $F_r$ is at most $7/8 < 1$,
	this lets us push the number of satisfying assignments down and report NO.
	
	Intuitively, this behavior (difference between $\rho$ bounded away from some power of two and just above a power of two by a tiny amount)
	makes sense: we know that GT-MAJ-3-SAT is hard
	for {\sf{\#P}}, so \thr{\rho}{3} should be much harder for $\rho = 1/2 + \eps$ 
	if we take $\eps$ sufficiently small (e.g. $\eps = \Omega(1/2^n)$), and this is reflected in the
	dependence of $q_t$ on $\rho - 1/2^{t+1}$, where $1/2^{t+1}$ is the largest power of two
	that is strictly smaller than $\rho$, in the above proof.
\end{remark}

%We also introduce a ``greater than'' version of this problem called \thr{>\rho}{$k$}, which is the task of deciding if strictly greater than a $\rho$-fraction of assignments to a $k$-CNF are satisfying. 
%In this section, we establish the complexity of these problems for constant $\rho$ and $k$ through the following two results.


(Below was moved from MAJORITY-SAT With One Extra Clause Proof)

\note{Is it hard to determine if $\#2SAT(F) \geq 2^i$ or not, for a given $i$? It may be a hard problem, but the proof is not clear to me, even though $\#2SAT$ is $\#\P$-hard. The known reductions from $\#3SAT$ to $\#2SAT$ seem to go through permanent; they radically change the number of SAT assignments. The proof that $\#3SAT(F) \geq 2^{n/2}$ is $\PP$-hard uses the fact that the reduction from Circuit-SAT to 3SAT is parsimonious. If we could prove that $\#2SAT(F) \geq 2^i$ is $\PP$-hard then the above proof would extend to $3$-CNF formulas with one clause of arbitrary width.}

\note{The problem seems to be related to whether determining if the permanent is at least $2^i$ or not. In a 0-1 matrix, computing the permanent corresponds to computing the number of perfect matchings in a bipartite graph. Valiant proceeds by reducing counting perfect matchings to counting \emph{all} matchings (not just perfect ones), but this reduction apparently requires making $n+1$ calls to an oracle for counting all matchings. \url{https://www.math.cmu.edu/~af1p/Teaching/MCC17/Papers/enumerate.pdf} The latter problem can be reduced to $\#2SAT$ by making an instance with a variable $x_i$ for the $i$-th edge, and the clauses $(\neg x_i \vee \neg x_j)$ for all pairs of edges $i,j$ with a common endpoint.}


\note{We know E-MAJ-3SAT is NP-complete. What about E-MAJ-2SAT? Partition clauses into three kinds: those with only vars from "first half", those with only vars from "second half", those with one var from each... for the clauses only over the "MAJ" variables we can either conclude UNSAT (because it has a large disjoint set) or that it can be expressed as an O(1)-size decision tree of 1-CNFs. So for E-MAJ-2SAT we want to find an assignment to the E vars such that the resulting "MAJ" decision tree has at least half SAT assignments. This must have a lot of structure. if we have $(x \implies y) \wedge (x \implies z)$ for distinct variables $y$ and $z$ which are MAJ variables, and $x$ which is an E variable, then $x$ must be false: otherwise there are two few SAT assignments. In general, we must find an assignment to the E variables which assigns at most one MAJ variable (so that the number of SAT assignments is at least half). Seems MAJ-MAJ-2SAT should be easy...}

%	*** 
%	
%	
%For $2$-CNF, the idea would be about the same as the one for E-MAJ2SAT below. For $3$-CNF, it is more complicated because there are more cases for the clauses: there are clauses containing only $x$-variables, clauses containing one $x$-variable and two $y$-variables, clauses containing two $x$-variables and one $y$-variables, and clauses containing only $y$-variables. I think it should be that each of these subformulas has a small maximal disjoint set. Clearly this has to be true for all-$x$-variable clauses and all-$y$-variable clauses when the fraction is $\geq 1/2+\eps$...
%***
%
%Perhaps, as with E-MAJ2SAT, we can try all small sets of literals and 2-clauses over the second set of variables, which correspond to subformulas that may be  ``forced'' by the first set of variables. But we would have to verify that a majority of the assignments to the first set actually leads to a majority of assignments to the second set being satisfying. ***


\begin{theorem}
	\label{thm:majmaj-2sat-linear}
	There is a deterministic linear time algorithm for \MAJMAJkSAT{$2$}.
\end{theorem}
\begin{proof}
    \snote{In progress\dots}
    Let $\vec{x} = (x_1, \dots, x_n)$ and $\vec{y} = (y_1, \dots, y_{n'})$ be the collections of \emph{outer} and \emph{inner} variables respectively.
    Take an arbitrary 2-CNF formula $\varphi = \varphi(\vec{x}, \vec{y})$ over the outer and inner variables.
    Then our task is to decide whether the inequality 
        \begin{equation}
        \label{eq:nest-prob-1/2}
        \Pr_{\vec{a}}\left[\Pr_{\vec{b}}[\varphi(\vec{x},\vec{y}) \mid \vec{x}=\vec{a}]\ge 1/2\right] \ge 1/2
        \end{equation}
    holds, where the outer probability is taken over a uniform random assignment to $\vec{a}$ to $\vec{x}$ and the inner probability is taken over a uniform random assignment $\vec{b}$ to $\vec{y}$.
    
    Partition the clauses of $\varphi$ into the set $C_x$ of clauses only on the outer variables, the set $C_y$ of clauses only on the inner variables, and the set $C_{xy}$ of clauses containing exactly one outer variable and one inner variable.
    
    Take a maximal disjoint set $S_x$ of clauses from $C_x$.
    If $|S_x| \ge \lceil\log_2(4/3)\rceil = 3$ we  return NO, since by \Cref{prop:subformula} the fraction of assignments to $\vec{x}$ which allow $\varphi$ to be satisfiable at all is at most $(3/4)^3 < 1/2$, so \cref{eq:nest-prob-1/2} cannot hold.
    Otherwise, $|S_X| \le 2$.
    
    Then take a maximal disjoint set $S_y$ of clauses from $C_y$.
    Similar reasoning shows that it if $|S_y| \ge 3$ is an return NO.
    Otherwise, assume that $|S_y| \le 2$.
    
    Now, 
    
\end{proof}



%Can even say: for any Boolean constraint problem on $n$ variables with constraints of width at most three, we can determine if it has at least $\alpha \cdot 2^n$ satisfying assignments. We can also determine if it has \emph{greater than} $\alpha \cdot 2^n$ satisfying assignments by adjusting the YES case to check if the resulting $2$-CNF is satisfiable or not.


For any integer $k$ and thresholds $\rho, \sigma \in (0,1)$, let THR$_{\rho}$-THR$_{\sigma}$-$k$SAT be the problem of deciding whether an input $k$-CNF formula $\varphi$ satisfies
\begin{equation}
\label{eq:nested-prob}
\Pr_{\vec{a}}\left[\Pr_{\vec{b}}[\varphi(\vec{x},\vec{y}) \mid \vec{x}=\vec{a}]\ge \sigma\right] \ge \rho.\end{equation}

For example, \textsf{THR}$_{1/2}$-\textsf{THR}$_{1/2}$-$k$SAT is just the \MAJMAJkSAT{$2$} problem.
We now show the following result, which can be viewed as an extension of the ideas from our threshold SAT algorithm for 3-CNF formulas given in the proof of \Cref{thm:thr-3-sat}.

\begin{theorem}
	\label{thm:majmaj-2sat-linear}
	Let $\rho, \sigma \in (0,1)$ be rationals whose denominators are bounded above by constants.
	Then there is a deterministic linear time algorithm for solving  \thrthr{\rho}{\sigma}{2}.
\end{theorem}
\begin{proof}
	Let $\vec{x} = (x_1, \dots, x_n)$ and $\vec{y} = (y_1, \dots, y_{n'})$ be the collections of \emph{outer} and \emph{inner} variables respectively.
	Take an arbitrary 2-CNF formula $\varphi = \varphi(\vec{x}, \vec{y})$ over the outer and inner variables.
	Our task is to decide whether inequality from \cref{eq:nested-prob} 
	holds, where the outer probability is taken over a uniform random assignment to $\vec{a}$ to $\vec{x}$ and the inner probability is taken over a uniform random assignment $\vec{b}$ to $\vec{y}$.
	
	Define $C_x$ to be the set of clauses in $\varphi$ containing only outer variables.
	We call this the set of \emph{outer clauses}.
	Also define $C_{xy}$ to be those clauses containing exactly one outer variable and one inner variable.
	We call this the set of \emph{mixed clauses}.
	
	Take a maximal disjoint set $S_x$ of clauses from $C_x$.
	Set $t_x =  \lceil\log_{4/3}(1/\rho)\rceil$.
	If $|S_x| > t_x $ we  return NO, since by \Cref{prop:subformula} the fraction of assignments to $\vec{x}$ which allow $\varphi$ to be satisfiable is at most $(3/4)^{t_x} < \rho$.
	Otherwise, $|S_x| \le t_x$.
	
	Set $t = \log_2(1/(\sigma\rho))$.
	Now, let $q_1 > q_2 > \dots > q_t$ be integer constants whose values we set later.
	Intuitively, these parameters will are the cutoffs for sizes of large 1-sunflowers among the mixed clauses, whose cores are inner variables.
	
	Initialize $r=0$.
	This will be a count for the number of 1-sunflowers we find.
	
	While $r\le t$, run the following procedure:
	\begin{itemize}
		\item 
		\item
		
	\end{itemize}
\end{proof}


%\begin{corollary}
%Given any Boolean CSP $F$ with constraints of arity at most three, we can determine in polynomial time if at least half of the assignments to $F$ are satisfying.
%\end{corollary}

%\begin{proof} Given such a CSP $F$, each constraint can be converted to a $3$-CNF formula in the natural way.
%We can then apply the above algorithm can then handle it.
%\end{proof}


%If we find a satisfying assignment, then we return YES because
%		    \[\Pr[\varphi] = \Pr[\varphi'] = \frac 12\cdot\grp{\Pr[\varphi'\mid \ell ] + \Pr[\tilde{\varphi}]} > 1/2.\]
%		 If we find no such satisfying assignment, then $\Pr[\varphi] = \Pr[\varphi'] = 1/2$ exactly so we return NO.
%		 \rnote{here we want to say ``if the guessed assignment does not satisfy for $\tilde{\varphi}$ then return NO.''}
%First, we nondeterministically guess a satisfying assignment to $\varphi\land\lnot\psi$. 
%If we guess such a satisfying assignment, then we can immediately return YES: we have
 %   \[\Pr[\varphi] = \Pr[\varphi\land\psi] + \Pr[\varphi\land\lnot \psi] > 1/2\]
%where the first summand is at least $1/2$ and the second summand is greater than $0$.
%Otherwise, if no satisfying assignment to $\varphi\land\lnot\psi$ is found, then $\Pr[\varphi] = \Pr[\varphi'] \ge 1/2$.
%In this scenario, we make another guess based on which of the above two cases we fall into.
%\begin{description}
%		\item[Case 1: Covered by a Literal] \hfill\\
%		Suppose every clause of $\varphi'$ contains a common literal $\ell$.
%		Let $\tilde{\varphi}$ be the formula formed by removing all occurrences of $\ell$ from $\varphi'$ (equivalently, we are setting $\ell$ to be false in $\varphi'$). Nondeterministically guess a satisfying assignment for $\tilde{\varphi}.$
%		If we find a satisfying assignment, then we return YES because
%		    \[\Pr[\varphi] = \Pr[\varphi'] = \frac 12\cdot\grp{\Pr[\varphi'\mid \ell ] + \Pr[\tilde{\varphi}]} > 1/2.\]
%		The last inequality follows from the observation that 
%		 $\Pr[\varphi'\mid \ell ] = 1$ because setting $\ell$ true automatically satisfies $\varphi'$, and $\Pr[\tilde{\varphi}] > 0$ from the satisfying assignment we found.
%		 If we find no such satisfying assignment, then $\Pr[\varphi] = \Pr[\varphi'] = 1/2$ exactly so we return NO.

%		\item[Case 2: Exact Count] \hfill\\
%		Suppose we have the exact fraction of satisfying assignments to $\varphi'$.
%		Then as noted before, $\Pr[\varphi] = \Pr[\varphi']$, so here we can simply return NO if the fraction of satisfying assignments equals exactly $1/2$, and otherwise (when the fraction is greater than $1/2$) we return YES.
%\end{description}




\begin{comment}	
	Given a Boolean formula $\Phi$, let $\Pr[\Phi]$ denote the probability a random assignment to the variables of $\Phi$ is satisfying.
	For a given $k$-CNF $\varphi$, we want to decide whether the inequality
			\[\Pr[\varphi] \ge \rho\]
	holds or not. 
	We will do this by building up a special $(k-2)$-CNF $\psi$ on the same variable set, where each clause of $\psi$ is contained in a clause of $\varphi$. We split the probability calculation into
	\[\Pr[\varphi] = \Pr[\varphi\land \psi] + \Pr[\varphi \land \lnot\psi].\]
	Recalling that $\Pr[\varphi\mid\lnot\psi] \geq \Pr[\varphi\wedge\lnot\psi]$, we observe
		\begin{equation}
		\label{eq:prob-bound}
		\Pr[\varphi\land\psi]\le \Pr[\varphi]\le \Pr[\varphi\land\psi] + \Pr[\varphi\mid\lnot\psi].
		\end{equation}
	%Here, the summand $\Pr[\varphi\mid\lnot\psi]$ denotes the fraction of assignments which satisfy $\varphi$ among those assignments to $\varphi$ which do not satisfy $\psi$.
	Intuitively, we will construct $\psi$ in such a way that 
	$\Pr[\varphi\mid\lnot\psi] < \eps_1$
	for an \emph{extremely} small $\eps_1 > 0$,
	so that it is possible to reduce the problem of determining $\Pr[\varphi] \geq \rho$ to the problem of determining $\Pr[\varphi\land\psi] \geq \rho$. In other words, we are reducing \thr{\rho}{$k$} on $\varphi$  to 
	\thr{\rho}{$k$} on $\varphi\land\psi$.

	This reduction is helpful because the clauses of $\psi$ are subclauses appearing frequently in $\varphi$, so the formula $\varphi\land\psi$ simplifies to a smaller formula.
	Additionally, adding the clauses of $\psi$ to $\varphi$ reduces the size of the solution space of $\varphi$, so intuitively it becomes easier to check if the resulting formula has fewer than a $\rho$-fraction of satisfying assignments.
	
	More precisely, \cref{eq:prob-bound} shows that if $\varphi\land \psi$ is a YES instance for \thr{\rho}{$k$} then we know $\varphi$ is a YES instance as well.
	The more surprising result is that we can construct $\psi$ in such a way that 
	if $\Pr[\varphi\land\psi] < \rho$, then (just as in our algorithm for \thr{\rho}{$3$}) we can in fact infer that $\Pr[\varphi\land\psi] < \rho - \eps_2$ for some $\eps_2 > \eps_1$.
	Hence by \ref{eq:prob-bound} we can deduce that $\Pr[\varphi] < \eps_1 + \rho - \eps_2 < \rho$.
	
	We construct the clauses of $\psi$ by taking cores of large sunflowers in $\varphi$. Defining what counts as ``large'' depends on quite a few parameters, so the analysis becomes technical. 
	\end{comment}
	
	
It is also possible to get a smaller upper bound on the asymptotic runtime when $\rho$ is dyadic (i.e. its denominator is a power of 2).
This is because in this case we can get a larger lower bound for $\eta$ by inspecting the proof of \Cref{lm:gen-bit-argument} from \Cref{sec:eff-parameter}, so we can take $q_t$ to be $O(\log(1/\rho))$ instead of $O(\log b)$.
This still leads to a tower of exponentials however.

% Comments removed from arxiv
	 
	 %	Let $q$ be the smallest positive integer such that 
	 %	\snote{This choice of $\beta$ works but might be more complicated than necessary\dots 
	 %	in particular maybe it suffices to work with $(1/2^{t_1})(1 - 1/2^k)$ on the left hand side instead (and get a simpler definition for $\beta$).}
	 
	 %			\[\frac{1}{2^{t_1}}\cdot \grp{1 - \frac{1}{2^k}} +
	 %			\grp{1 - \frac{1}{2^{t_1}}}\grp{1 - \frac{1}{2^{k-1}}}^q < \rho.\]
	 
	 %	Such a $q$ exists because the we took $t_1$ with $\rho\ge (1/2)^{t_1}$.
	 %	Now set 
	 %	
	 %		\[\beta = \rho - \frac{1}{2^{t_1}}\cdot \grp{1 - \frac{1}{2^k}} +
	 %		\grp{1 - \frac{1}{2^{t_1}}}\grp{1 - \frac{1}{2^{k-1}}}^q >0 \]
	 
	 
%\def\P{{\mathsf{P}}}


% \newcommand{\majsat}[1]{{{\textsf{MAJ-{#1}SAT}}}

%%% Other title possibilities:
% Majority-SAT on k-CNFs in Deterministic Linear Time (via Sunflowers)
% Majority-k-SAT in P
% Solving Threshold SAT on Bounded Width Formulas in Deterministic Polynomial Time
% Separating Complexities of Majority-SAT and Majority-k-SAT
%%%
%\title{Algorithms and Hardness for\\ Threshold Counting Problems over $k$-CNF Formulas
	 
%Solving MAJORITY-SAT on kCNFs with Sunflowers}

%\footnote{Strictly speaking, $\#SAT(F) \geq 2^{n-1}$ determines the ``highest-order'' bit only when $\#SAT(F) < 2^n$ and we output $n$ bits. Otherwise, $\#SAT(F) \geq 2^{n-1}$ is the OR of the two highest-order bits. (When we output $n+1$ bits, the highest-order bit indicates whether or not $\#SAT(F)=2^n$, which is $\mathsf{coNP}$-complete.) Nevertheless,
%Thinking of \MAJSAT\ as the ``high-order bit of $\#SAT$'' is useful intuition for understanding its power, and for comparing with problems such as PARITY-SAT.

 %} 
%For simplicity, we just refer to this OR of two high-order bits as the ``high-order bit,'' as it does equal the high-order bit when $\#SAT(F)<2^n$ and $\#SAT(F)$ is $n$ bits long.}

% PARITY-SAT is complete for the class $\oplus P$~\cite{ValiantParity}, while MAJORITY-SAT is complete for the class $\PP$~\cite{prob-simon,prob-gill}. 

%, in stark contrast to the low-order bits which are $\NP$-hard.\footnote{The low-order bits correspond to computing $\oplus kSAT$, which cannot be computed in randomized polynomial time unless the polynomial hierarchy is in $\BPP$. This is true even for $k=2$~\cite{ValiantParity}.} %: they can be computed in polynomial time. 

%Intuitively, in \EMAJSAT, we want to know if there is a way to assign the first $k$ variables of $\phi$ so that a majority of the remaining assignments satisfy $\phi$ (corresponding to the design of some object that makes a condition hold with good probability). 

%\begin{theorem} \label{majmaj3SAT-linear-time} \MAJMAJkSAT{3} is in linear time.

%Our results imply that, \emph{for $3$-CNF formulas}, E-MAJSAT is in fact $\NP$-complete, contradicting several claims in the literature that this special case was also $\NP^{\PP}$-complete. 

% A disjoint set of clauses can be viewed as a sunflower with an empty core; a set of clauses which all contain a single common variable may also be useful in estimating the fraction of satisfying assignments. To give a simple example, if the entire formula was a sunflower with a single literal $\ell$ in its core, then the fraction of satisfying assignments is at least $1/2$ (because setting $\ell$ true already satisfies the formula). 

%At a very high level, the strategy behind our algorithms is to look for particular small subformulas $F'$ of a given $F$ where the fraction of assignments satisfying $F'$ is already less than $\rho$. 
%When such subformulas $F'$ exist, we can conclude that $\#SAT(F) < \rho \cdot 2^n$. 
%When these subformulas do not exist, this imposes further structure on $F$ that we can exploit in our algorithm.

%In fact, our hardness results imply that, even for CNFs with only one unbounded-width clause, such algorithms cannot be used to solve \MAJSAT\ unless $\P=\NP$.

%This restriction on what sorts of count can be produces is the main addition to previous work that allows us to solve threshold counting problems.

% to be the smallest integer such that $(3/4)^{c(\alpha)} < \alpha$. 

% and it can be efficiently computed.


%Note that we can also use the same algorithm to show that \GMAJkSAT{$k$} is in linear time. The 

%\footnote{Indeed, inspecting the proof of \Cref{thm:maj2sat}, one can verify that determining the high-order bits of $\#2SAT$ can even be done in $\mathsf{AC}^0$: The circuit can try all $m^{O(K)}$ subsets $S$ of $K$ clauses for a sufficiently large constant $K$; if some $S$ is disjoint, the circuit outputs $0$, otherwise the circuit tries all $3^K$ satisfying assignments to the given $S$, checks that what remains is $1$-CNF, and solves the resulting $\#1SAT$ instance if the check passes. 
%All this can be done in $\mathsf{AC}^0$.}

%The problem of deterministically finding a satisfying assignment to a formula with many satisfying assignments has been explored by several researchers, as it is a natural pseudorandomness question
%\cite{AtWig, Hirsch_detsat, Trevisan04, SerTan}: when there are at least $2^{n-\eps n}$ satisfying assignments, we expect one of $O(2^{\eps n})$ uniform random assignments to be satisfying. As one example, \cite{Trevisan04} shows how to find satisfying assignments to $k$-CNFs in *** time when there are at least ***. \Cref{thm:maj2sat} shows that for 2-CNFs, one can also \emph{exactly count} satisfying assignments when there are many.

%\begin{corollary} For every $2$-CNF $F$ with at least $2^{n-\eps n}$ satisfying assignments, the number of satisfying assignments can be  counted exactly in $O(m \cdot 2^{3.82 \eps n})$ deterministic time. 
%\end{corollary}


%{\bf Algorithm A.} \emph{(With two unspecified constants $c_1$ and $c_2$.)}\\
%\noindent 1. Given a 3-CNF $F$, find a maximal disjoint set $S$ of clauses of $F$.\\
%2. If $|S|$ exceeds a certain constant $c_1$, then output {\bf NO}.\\
%3. For all $7^{|S|}$ SAT assignments $A$ to the clauses in $S$,\\ 
%\indent ~~~ 3a. Let $F_{A}$ be the $2$-CNF induced by assignment $A$.\\
%\indent ~~~ 3b. Search for a maximal disjoint set $S_{A}$ of 2-clauses in $F_{A}$.\\
%\indent ~~~ 3c. If $|S_{A}|$ exceeds a certain constant $c_2$, then output {\bf NO}.\\
%\indent ~~~ 3d. Otherwise, try all SAT assignments $A'$ to the clauses in $S_A$.\\
%\indent ~~~~ For each $1$-CNF formula induced by an $A'$, count solutions to the $1$-CNF in polynomial time.\\
%4. Return {\bf YES} if and only if the total number of solutions counted is at least $2^{n-1}$.


 %What we prove below is slightly more general than what is required (we consider the case of arbitrary $k$, rather than $k=3$).
 
 %In the previous subsection, we showed how Threshold-3SAT can be solved for all threshold values $\rho > 1/2$. 
 
 
%Digging into the analysis, we see that the above algorithm can be modified to determine if a $3$-CNF has at least $\alpha 2^n$ satisfying assignments for any constant $\alpha > (7/8)\cdot 1/2 = 7/16$, by setting the parameter $t$ in Lemma~\ref{lemma:subformula1} to be sufficiently large.

% 		Now, by casework on which of the $\ell_i$ are set to true we see that $\ssat{\varphi}$ is equal to 
% \[		    \ssat{\varphi\land \lnot \ell_1} + \ssat{\varphi\land \ell_1\land\lnot \ell_2} + \dots + \ssat{\varphi\land \ell_1\land\dots\land \ell_{r-1}\land\lnot\ell_r} + \ssat{\varphi\land \ell_1\land\dots\land\ell_r}.\]

% 		In the above sum, the first $r$ addends together count the satisfying assignments which set some $\ell_i$ to be false.
% 		The final term counts the satisfying assignments which set all the $\ell_i$ to be true.
			
% 		Using \Cref{obs:3sun-small} to bound the first $r-1$ terms in the above sum, we deduce that
		
% 			\[\ssat{\varphi} \le 
% 			\grp{\frac 12\cdot \grp{\frac 34}^{q_0} + \dots + \frac 1{2^r}\cdot \grp{\frac 34}^{q_{r-1}}}2^n
% 			 + N < \grp{1 - \frac 1{2^r}}\grp{\frac 34}^{q_{r-1}}2^n + N\]
			
% 		by considering which of the $\ell_i$ are set to false under possible assignments.
		
% 		Thus, if we pick $q_{r-1}$ large enough that 
% 			\[
% 			\grp{\frac 34}^{q_{r-1}} \le \frac{\eta}{1 - (1/2)^r}
% 			\]

				
%					\item 
%					\label{step:1-sun}
%						Suppose instead step 2\ref{step:gen-sun} outputs a 1-sunflower of size at least $Q_1$.
%						
%						Let $S$ be this sunflower and $C = \set{\ell}$ be its core consisting of a single literal $\ell$.
%						
%						Update formula $\psi\leftarrow \psi\land \ell$.
%						
%						Let $F'$ be the formula obtained from $F$ by removing all clauses of $F$ containing $\ell$.
%						
%						Update $F\leftarrow F'\land \ell$.
%						
%						\textcolor{Gray}{~ This corresponds to asserting that $\ell$ is true.}
%						
%						Increment $r\leftarrow r+1$.
%						
%						Reset $r_w\leftarrow 0$ for $2\le w\le k-2$.
%						
%					\textcolor{Gray}{~ We update the counts since we found a new 1-sunflower.}
					
%					\item 
%					\label{step:w-sun}
%						Suppose instead step 2\ref{step:gen-sun} returns a $w$-sunflower with weight $w\ge 2$.
%						
%						Let $S$ be this sunflower and $C$ bits core, viewed as a clause on $w$ literals.
%						
%						For each literal $\ell$ in $C$, check if $F$ contains a 1-sunflower of size $Q_1 = q_1(r)$
%						with $\ell$ as its core.
%						If such a sunflower exists, go to step 2\ref{step:1-sun} and run it with this sunflower instead.
%
%						\textcolor{Gray}{
%							~ The above check ensures that whenever we add a sunflower of weight greater than 1,
%							none of its literals belong to a large 1-sunflower.
%						This helps us later bound the number of times any literal appears in $\psi$, which will be useful in the proof of correctness.}
%
%						
%						Otherwise, update formula $\psi\leftarrow \psi\land C$.
%						
%						Increment $r_w \leftarrow r_w+1$.
%						
%						Let $F'$ be the formula obtained by removing every clause of $F$ which contains $C$ as a subclause.
%						Update $F\leftarrow F'\land C$.
%						
%						\textcolor{Gray}{~ As in step 2\ref{step:1-sun}, this final step corresponds to asserting that $C$ is true in $F$.}


% 		if an assignment to the variables of $\varphi$ does not satisfy some clause $C$ of $\psi$, to be satisfying for $\varphi$ it must satisfy the variable disjoint set of clauses formed by removing core $C$ from its corresponding sunflower $S$.

% 		Furthermore, suppose the clause $C$ was added in 
% 		the algorithm when the variable $\vec{r}$ had the particular value $\vec{r}(C) = (r_1(C), \dots, r_{k-2}(C))$.

	%	The formula $D_i$
%	 is true if and only if $C_i$ is not satisfied and all $C_j$ are satisfied where $j < i$.

		
%		We pick the $q_1(s)$ so large that 
%		
%			\begin{equation}
%			\label{eq:1-sun-growth}
%			\grp{1 - \frac{1}{2^{k-1}}}^{q_1(s)} < \eta
%			\end{equation}
%			
%		for all $s<r$.
%		This just means that $q_1(s)$ is sufficiently large as a function of the $q_1(r)$ for $r>s$ and all the  $q_w(\vec{r})$ for which $\vec{r}= (r, r_2, \dots, r_{k-2})$ has $r>s$.
%		
%		Similarly, each clause of width $w \ge 2$ in $\psi$ has size $q_w(\vec{s})$ 
%		where $\vec{s} = (s, s_2, \dots, s_{k-2})$ either has
%		
%			\[s < r\]
%		
%		or has
%		
%			\[s = r \quad \text{and} \quad s_w < r_w.\]
%			
%		Then we make sure to pick values of the $q_w(\vec{s})$ so large that 
%		
%			\begin{equation}
%				\label{eq:w-sun-growth}
%				\grp{1 - \frac{1}{2^{k-w}}}^{q_w(\vec{s})} < \eta.
%			\end{equation}
%		
%		Similar to the 1-clause case, this happens provided we take $q_w(\vec{s})$ to be a large enough function of the  $q_1(r)$ with $r>s$ and the $q_v(\vec{r})$ over all $v\ge 2$ whenever $\vec{r} = (s, r_2, \dots, r_{k-2})$ has $r_w > s_w$ and $r_{u} \ge s_{u}$ for $u\neq w$.

% 		Now let $A$ be an arbitrary integer. 
% 		Suppose $S_\ell$ contains at least
% 			\[2(w-1)P\cdot A + 1\]
% 		clauses.
% 		Among these clauses, we construct a maximal variable disjoint set by greedily selecting clauses that share no variables with the clauses we have already picked.
% 		Call clauses that we cannot pick \emph{eliminated}.
		
% 		Each time we take a clause, at most $2(w-1)P$ other clauses are eliminated, since a given clause shares variables with at most $2(w-1)$ literals, and each such literal appears in at most $P$ clauses by the inductive hypothesis. 
% 		Consequently, given $2(w-1)P\cdot A + 1$ starting clauses, the greedy algorithm recovers a variable disjoint set of size at least $A+1$.
		
% 		Then if we set $A = Q_1-1$, we see that if $S_\ell$ has at least
		
% 			\[2(w-1)P\cdot A + 1 = (w-1)!\cdot 2^{w-1}\prod_{k=1}^{w-1}\grp{Q_k-1} + 1\]
% 		clauses, $S_\ell$ will have a 0-sunflower of size $Q_1$.
% 		This pulls back to a 1-sunflower of the same size in $S$,
% 		which contradicts the condition from \Cref{claim:bounded-repetition}.
% 		But the size of $S_\ell$ is just the number of times $\ell$ appears in $\psi'$.
% 		Thus it must be the case that actually $\ell$ appears at most 
% 			\[(w-1)!\cdot 2^{w-1}\prod_{k=1}^{w-1}\grp{Q_k-1} \]
% 		times, which completes the induction and proves the desired result.

%\begin{proof}
%	Let $\vec{x} = (x_1, \dots, x_n)$ be the list of \emph{outer variables} and $\vec{y} = (y_1, \dots, y_{n'})$ be the list of \emph{inner variables}.
%	Then given an arbitrary 3-CNF $\varphi = \varphi(\vec{x}, \vec{y})$ over all of these variables, 
%	the formula is a YES instance for the \MAJMAJkSAT{$3$} problem if and only if the inequality
%	
%	\[	
%		\Pr_{\vec{x}}\left[ \Pr_{\vec{y}} \left[\varphi(\vec{x}, \vec{y}) \right] \ge 1/2  \right] \ge 1/2
%	\]
%	holds, where the probabilities are taken with respect to uniform random Boolean assignments to the relevant variables.
%	To help check whether this inequality holds, we use the following observation.
%	
%	\begin{claim}
%		\label{claim:maj-avg}
%		For any formula $\varphi$ and threshold $\rho \in (0,1)$, if
%			\[\Pr_{\vec{x}, \vec{y}}\left[\varphi(\vec{x}, \vec{y})\right] < \rho\]
%		then we also have
%			\[\Pr_{\vec{x}}\left[ \Pr_{\vec{y}} \left[\varphi(\vec{x}, \vec{y})  \right] \ge 1/2 \right] < 2\rho.\]
%	\end{claim}
%		\begin{proof}
%			We prove the contrapositive.
%			Suppose that 
%						\[\Pr_{\vec{x}}\left[ \Pr_{\vec{y}} \left[\varphi(\vec{x}, \vec{y})  \right] \ge 1/2 \right]\ge 2\rho.\]
%						
%			This means for at least a $2\rho$ fraction of the assignments to the variables $\vec{x}$, we get a formula which is satisfied by at least $1/2$ of all assignments to variables in $\vec{y}$.
%			But assigning values to the variables in $\vec{x}$ and then $\vec{y}$ is the same as assigning values to all the variables, so we have 
%				\[\Pr_{\vec{x}, \vec{y}}\left[\varphi(\vec{x}, \vec{y})\right] \ge 2\rho \cdot \frac 12 = \rho\]
%			as desired.
%		\end{proof}
%	
%	We now describe the algorithm for \MAJMAJkSAT{$3$}.
%	
%	First, run the algorithm from \Cref{thm:thr-3-sat} to solve 
%	\thr{1/4}{3} on $\varphi$.
%	Recall this algorithm is parameterized by an integer $z$ corresponding to the size of a 0-sunflower it seeks, and two integers $q_1 > q_2$ corresponding to the sizes of $1$-sunflowers it searches for. 
%	the algorithm runs in linear time provided these parameters are all bounded above by constants.
%	
%	If the algorithm returns NO then by \Cref{claim:maj-avg} we can immediately return NO for the \MAJMAJkSAT{$3$} problem as well.



%\subsection{Discussion}

%The above result appears to be a ``barrier'' for algorithms solving MAJ4SAT. 


%\url{https://www.cs.utexas.edu/users/diz/Sub%20Websites/Research/On_unapproximable_versions_np_complete_problems.pdf}
%	\url{https://epubs.siam.org/doi/pdf/10.1137/S0097539797321602}

%For simplicity, we will just consider the case of deciding whether the number of SAT assignments is at least $2^{n-1}$, but the argument 


%Suppose we simply ignored the arbitrary width clause in our algorithm, and our algorithm proceeds by searching for various structured $4$-CNF subformulas. If they exist then we report NO,  otherwise we branch on their assignments, etc, until we get 1cnfs. If we then ``add back'' the arbitrary width clause into the 1cnfs, we can still solve $\#SAT$ for each (1cnf + long clause) in polynomial time, by simply resolving the unit clauses with the long clause. Thus in those cases we can still count the satisfying assignments exactly.

%This argument appears to show that MAJ2SAT with one arbitrary width clause (even $O(\log n)$ arbitrary width clauses) is decidable in $\P$.

%What happens when we try to apply our MAJ3SAT algorithm to solve MAJ3SAT with one arbitrary width clause? The only YES case we have to worry about is where every clause contains the same variable, which we can of course check for the arbitrary width clause as well. However, after the YES case fails, we are looking for a group of 3-clauses that all contain a popular literal, along with at least one extra clause that does not contain that literal. (This is Lemma~\ref{lemma:subformula1}.) 
%If that extra clause in Lemma~\ref{lemma:subformula1} is of arbitrary length, then the fraction of satisfying assignments is less than $1/2((3/4)^t + (1-1/2^w))$, where $w$ is the width of our long clause. If for example, $t = \Omega(n)$, then this fraction is $1/2 + 1/2 \cdot (3/4)^t - 1/2^{w-1}$, so this case will not apply (and answer NO) if $1/2 \cdot (3/4)^t \geq 1/2^{w-1}$. Thus Lemma~\ref{lemma:subformula1} doesn't apply when $w$ is large and our one extra clause is long! Any polytime algorithm for MAJ4SAT must have a similar property.

    % \begin{itemize}
    % \item
    % First, for each index $i$, $F_i$ is precisely the set of clauses of $\varphi$ which contain $\ell_i$, but are not in any of the $F_j$ for any $j<i$.
    % \item 
    % Second, $\varphi'$ has a constant size maximal disjoint set $S$.
    % Moreover, for any assignment $A$ to $S$, the formula $\varphi'_A$ induced from $\varphi$ by setting values according to $A$ also has a constant size maximal disjoint set.
    % This is equivalent to saying that $\varphi'$ can be represented as a constant size decision tree with 1-CNFs at the leaves.
    % This decision tree representation is already computed by the \thr{\rho}{3} algorithm.
    % \item
    % Third, we know that $\Pr[\varphi']\ge \rho$.
    % \item
    % Fourth and finally, the satisfying assignments to $\varphi'$ are precisely the satisfying assignments to $\varphi$ which set $\ell_1, \dots, \ell_t$ to be true.
    % \end{itemize}
    
    
% %%
% In fact, we prove the following more general result.
% %%

%It is possible that this is the only ``difficult'' case of \GMAJkSAT{$4$}. If it is (and GT-MAJ-4-SAT is in $\P$ when, for every variable, there is at least one clause that does \emph{not} contain it) then GT-MAJ-4-SAT is actually $\NP$-complete: we check if there is a variable in all clauses. If so then we guess a SAT assignment for the resulting $3$-CNF; if not then we decide the problem in $\P$. This would also strongly suggest that this variant is not $\PP$-complete. (Otherwise, $\P^{\#\P}= \NP$.)

% 	\item {\bf Determine the complexity of \MAJkSAT{$3$} with one arbitrary-width clause.} 
% 	We showed that solving Majority-SAT on the conjunction of a $k$-CNF and an arbitrary width clause is $\NP$-complete for $k\ge 4$.
% 	The complexity for the $k=3$ case remains open however. 
% 	The complexity of this problem seems to boil down to whether checking $\#SAT(F) \geq 2^t$ is $\PP$-hard for $2$-CNFs and arbitrary integers $t$, or not. It is quite possible this problem is $\PP$-complete, but we have not yet encountered a proof.
	
